Pareto Optimal Strategies for Event-Triggered Estimation

Although resource-limited networked autonomous systems must be able to efficiently and effectively accomplish tasks, better conservation of resources often results in worse task performance. We specifically address the problem of finding strategies for managing measurement communication costs between agents. A well understood technique for trading off communication costs with estimation accuracy is event triggering (ET), where measurements are only communicated when useful, e.g., when Kalman filter innovations exceed some threshold. In the absence of measurements, agents can use implicit information to achieve results almost as well as when explicit data is always communicated. However, there are no methods for setting this threshold with formal guarantees on task performance. We fill this gap by developing a novel belief space discretization technique to abstract a continuous space dynamics model for ET estimation to a discrete Markov decision process, which scalably accommodates threshold-sensitive ET estimator error covariances. We then apply an existing probabilistic trade-off analysis tool to find the set of all optimal trade-offs between resource consumption and task performance. From this set, an ET threshold selection strategy is extracted. Simulated results show our approach identifies non-trivial trade-offs between performance and energy savings, with only modest computational effort.

==> sections/evaluation.tex <==

In this section we demonstrate the benefits of trade-off analysis by showing that small sacrifices in task performance can lead to large energy savings. We present Pareto Fronts for a 2D and 3D system generated using PRISM-games, \cite{Kwiatkowska2013}, and simulate specific strategies for interesting points. We simulated multiple points from each system and trajectory to compare the theoretical values for the objectives (obtained through analysis on the MDP) to the empirical results for the objectives (from 3000 simulations of the strategies). In all cases for the 2D system, we found the error between theory and simulation to be less than 2\%, and for the 3D system we found the error to be less than 3.5\%. 

\subsection{2D System}
We consider the system from \cite{Bry2011}, with dynamics:
\begin{align}
\label{eq:2Ddynamics}
    x_{k+1} &= x_k + u_k + w_k \\
    y_k &= x_k + w_k
\end{align}
with process noise $w_k \sim \mathcal{N}(0,0.07^2I)$ and measurement noise $v_k \sim \mathcal{N}(0,0.03^2I)$. For clarity, the communication cost is $c_m=1$ so that the energy is simply the raw number of triggers.

We first consider a winding trajectory through a set of obstacles, shown in Figure \ref{superGPP1}. For this trajectory, we built an MDP using both of the two abstraction methods described above. The resulting Pareto fronts are shown in Figure \ref{PPfrontCompMethods}. Note that due to the size of the MDP in the Discretized Belief Method, the Pareto Front is very complex, and Figure \ref{PPfrontCompMethods}.a. shows only a selection of interesting points. On the other hand, the simplicity of the MDP for the Enforced Belief Convergence Method allows for fast and easy computation of all vertices describing the full front, shown in Figure \ref{PPfrontCompMethods}.b..

\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.23\textwidth}
    \centering
        \includegraphics[width=\textwidth]{Set49ParetoFront.pdf}
        \caption{Discretized Belief Method}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
    \centering
        \includegraphics[width=\textwidth]{Set52ParetoFront.pdf}
        \caption{Enforced Belief Convergence Method}
    \end{subfigure}
    \caption{Pareto Fronts for 2D system with winding trajectory.}
    \label{PPfrontCompMethods}
\end{figure}

Each front shows a characteristic shape; from the highest probability of target there is a steep drop-off in energy which eases as the probability of target gets lower. This indicates relatively large energy savings for the highest probability of target, with smaller gains as the probability of target goes to its minimum. This shape is common across every Pareto Front generated in these studies, and supports the argument that this kind of analysis can provide valuable energy savings for little sacrifice in performance objectives. 

The second note from these two fronts is the contrast between the two methods. At the highest energy consumption, both methods offer similarly high probability of reaching the target ($98.8\%$ for the KF Convergence Method vs. $96.8\%$ for the Discretized Belief Method). However, the discretized belief method drops off to far lower values than the KF convergence method, indicating that method is better able to leverage ET and provide greater energy efficiency. 

\begin{table}[h!]

    \begin{center}
    \caption{3 Pareto Points for winding trajectory using the Discretized Belief Method}
    \label{tab:2Dwinding}
    \begin{tabular}{|| c | c | c | c ||}
    \hline
    Pareto Point & $P_{tar}$ & $P_{col}$ & $E_c$ \\
    \hline
         1 & 96.85\% & 3.14\% & 367.99 \\
         2 & 95\% & 4.70\% & 185.07 \\
         3 & 83.5\% & 14.68\% & 92.35 \\
         Full KF & 95.67\% & 3.97\% & 682.32\\
    \hline
    \end{tabular}
    \end{center}
\end{table}

To more closely examine interesting trade-offs for the Discretized Belief Method, consider Table \ref{tab:2Dwinding}, which shows 3 selected Pareto Points of interest in addition to expected performance if a regular KF is used at every time step. Pareto Point 1 is the point on the front with the highest probability of reaching the target. Pareto point 2 sacrifices only $1.8\%$ probability of target, but uses half the energy. However, Pareto Point 3 represents another halving of the energy, but the probability of target drops by $11.5\%$: the strength of the trade-off decreases as the energies become lower. Also note the stark comparison with the full KF performance; at its highest probability of reaching the target, ET achieves the similar performance for $54\%$ the energy use. The behaviors of the three Pareto Points can be seen in the simulation of their corresponding strategies, shown in Figure \ref{TrajectoryComp}.

\begin{figure}[b]
     \centering
     \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220302set49mergedMDPpp2.pdf}
         \caption{Pareto Point 1}
         \label{superGPP1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220302set49mergedMDPpp14.pdf}
         \caption{Pareto Point 2}
         \label{superGPP2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.13\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220302set49mergedMDPpp31.pdf}
         \caption{Pareto Point 3}
         \label{superGPP3}
     \end{subfigure}
          \hfill
     \begin{subfigure}[b]{0.07\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/colorbar.pdf}
         \label{superGPP3}
     \end{subfigure}
 
    \caption{Simulated strategies of three Pareto points for a 2D system using the Discretized Belief method. The color of the trajectory indicates $\bar{\gamma}(\delta)$ %the triggering threshold, $\delta$, chosen 
    for the $\delta$ chosen at each waypoint.}
    \label{TrajectoryComp}
\end{figure}

Figure \ref{TrajectoryComp} shows 300 simulated runs of each strategy, where the color of the trajectory indicates the triggering threshold. Each threshold can be directly mapped to an expected triggering rate (see \cite{Wu2013}). In the figure, cyan corresponds the highest expected triggering rate (100\%) and magenta the lowest (5\%). The efficiency of the strategies can be seen in how the triggering rate only increases (lower $\delta$) in proximity to obstacles, and otherwise relaxes (higher $\delta$) in more open parts of the trajectory. Higher triggering rates lead to a contraction in the trajectories, and therefore lower probabilities of collision. Trivially, we can see that the lower energy Pareto points correspond to lower triggering rates around the obstacles. 


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Set54ParetoFront.pdf}
         \caption{Pareto Front}
         \label{openPfront}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220307set54mergedMDPpp2.pdf}
         \caption{Pareto Point 1}
         \label{openPP1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220307set54mergedMDPpp6.pdf}
         \caption{Pareto Point 2}
         \label{openPP2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.07\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/colorbar.pdf}
     \end{subfigure}
        \caption{Pareto front and 2 simulated strategies for 2D System, open trajectory, using discretized belief method.}
        \label{openTrajectory}
\end{figure}

The Pareto front is specific to the trajectory chosen, and different trajectories yield different trade-offs. To demonstrate this, we consider a more open trajectory for the same 2D system with the Discretized Belief Method. This trajectory does not collide with any obstacles. The resulting Pareto Front and trajectories for two simulated points are shown in Figure \ref{openTrajectory}. Performance of the objectives for the two simulated Pareto points is shown in Table \ref{tab:2Dopen}.
\begin{table}[h!]
\begin{center}
    \caption{Two Pareto Points for open trajectory with Discretized Belief Method}
    \label{tab:2Dopen}
    \begin{tabular}{|| c | c | c | c ||}
    \hline
    Pareto Point & $P_{tar}$ & $P_{col}$ & $E_c$ \\
    \hline
         1 & 97.66\% & 0.0 & 52.58 \\
         2 & 95\% & 0.0 & 30.95\\
         Full KF & 97.43\% & 0.0 & 332.82\\
    \hline
    \end{tabular}
\end{center}
\end{table}

Note that because this trajectory avoids proximity with obstacles, the only difference in the Pareto Points comes at the very end of the trajectory going into the target region. Because there is really only one waypoint with a relevant action choice, the trade-offs between Pareto points are far less dramatic than the first trajectory, however the contrast with a using a full KF at every time step is amplified.


\subsection{3D System}
Finally, to demonstrate the flexibility of our abstraction method, we consider the same system as (\ref{eq:2Ddynamics}), but extended to three dimensions. A selection of interesting Pareto Points and a single simulated strategy for a winding trajectory using the Discretized Belief Method is shown in Figure \ref{3DTrajectory}. Note that the same general shape of the Pareto front holds for the 3D system, with generous trade-offs at higher energies that taper as the energy decreases. The simulated trajectory corresponds to the highest probability of target and shows similar behavior to the 2D system, with higher triggering rates closer to the obstacles.


\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Set53ParetoFront.pdf}
         \caption{Pareto Front}
         \label{3DPfront}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220307set53mergedMDPpp2View5.pdf}
         \caption{Pareto Point 1}
         \label{3DPP1}
     \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.07\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/colorbar.pdf}
    % \end{subfigure}

        \caption{(a) Pareto front and simulated strategy for 3D System; (b) `Super G' trajectory, using discretized belief method. } 
        \label{3DTrajectory}
\end{figure}

% evaluation.tex

==> sections/evaluationFinal.tex <==

Here, we demonstrate the benefits of trade-off analysis by showing that small sacrifices in task performance can lead to large energy savings. 
We present Pareto Fronts for a 2D and 3D system and simulations of strategies of interesting points. 
% We simulated multiple points from each system and trajectory to compare the theoretical values for the objectives (obtained through analysis on the MDP) to the empirical results for the objectives (from 3000 simulations of the strategies). 
In all cases, the error between theory and simulation was less than 2\% for the 2D and less than 3.5\% for 3D system. 
For more case studies and detailed discussions see \cite{Theurkauf2022}.

\paragraph*{2D System}
We considered the robotic system from \cite{Bry2011} with dynamics
\vspace{-2mm}
\begin{align}
\label{eq:2Ddynamics}
    x_{k+1} = x_k + u_k + w_k, \quad
    y_k = x_k + w_k,
\end{align}
where $w_k \sim \mathcal{N}(0,0.07^2I)$ and $v_k \sim \mathcal{N}(0,0.03^2I)$. For clarity, the communication cost is $c_m=1$ so that the energy is simply the raw number of triggers.
We considered a trajectory through a set of obstacles as shown in Figure \ref{superGPP1}. For this trajectory, we built an MDP using both of the two abstraction methods described above. The resulting Pareto fronts are shown in Figure \ref{PPfrontCompMethods}.
% Due to the size of the MDP in the Discretized Belief Method, the Pareto Front is very complex, and Figure \ref{fig:PPfrontSetMethod} shows only a selection of interesting points. On the other hand, the simplicity of the MDP for the Enforced Belief Convergence Method allows for fast and easy computation of all vertices describing the full front, shown in Figure \ref{PPfrontCompMethods}.b..


\begin{figure}[t]
     \centering
     \begin{subfigure}{0.125\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220302set49mergedMDPpp2.pdf}
         \caption{Pareto Point 1}
         \label{superGPP1}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.125\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220302set49mergedMDPpp14.pdf}
         \caption{Pareto Point 2}
         \label{superGPP2}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.125\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220302set49mergedMDPpp31.pdf}
         \caption{Pareto Point 3}
         \label{superGPP3}
     \end{subfigure}
          \hfill
     \begin{subfigure}{0.06\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/colorbar.pdf}
         \label{superGPP3}
     \end{subfigure}
 
    \caption{Simulated strategies of three Pareto points for the 2D system using the Discretized Belief method. The color of the trajectory indicates 
    % $\bar{\gamma}(\delta)$ 
    the expected triggering rate.
    % , $\delta$, chosen for the $\delta$ chosen 
    % at each waypoint.
    }
    \label{TrajectoryComp}
    \vspace{-1mm}
\end{figure}
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.235\textwidth}
    \centering
        \includegraphics[width=.97\textwidth]{Set52ParetoFront.pdf}
        \caption{Enforced Belief Convergence}
        \label{fig:PPfrontEnforcedMethod}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.235\textwidth}
    \centering
        \includegraphics[width=\textwidth]{Set49ParetoFront.pdf}
        \caption{Discretized Belief}
        \label{fig:PPfrontSetMethod}
    \end{subfigure}
    \caption{Pareto Fronts for 2D system with winding trajectory.}
    \label{PPfrontCompMethods}
    \vspace{-3mm}
\end{figure}

Each front shows a characteristic shape;  relatively large energy savings are achievable for the highest probabilities of reaching the target, with smaller savings as the probability of target goes to its minimum. This shape is common across every Pareto Front generated in these studies, and supports the argument that this kind of analysis can provide valuable energy savings for little sacrifice in performance objectives. 

The second note from these two fronts is the contrast between the two methods. At the highest energy consumption, both methods offer similarly high probability of reaching the target. However, the discretized belief method drops to far lower energy values than the KF convergence method, indicating that method is better able to leverage ET and provide greater energy efficiency. 

To more closely examine interesting trade-offs for the Discretized Belief Method, consider 
% Table \ref{tab:2Dwinding}, 
the table below.
It shows 3 selected Pareto Points of interest in addition to expected performance if a regular KF is used at every time step. 
\begin{table}[h]
    \begin{center}
    % \caption{3 Pareto Points of the Discretized Belief Method}
    % \label{tab:2Dwinding}
    \vspace{-2mm}
    \begin{tabular}{| c |  c   c   c |}
    \hline
    Pareto Point & $P_{\tar}$ & $P_{\coll}$ & $E_c$ \\
    \hline
         1& 0.969 & 0.031 & 367.99 \\
         2 & 0.950 & 0.047 & 185.07 \\
         3 & 0.835 & 0.147 & 92.35 \\
         Full KF & 0.957 & 0.397 & 682.32\\
    \hline
    \end{tabular}
    \end{center}
    \vspace{-4mm}
\end{table}

\noindent
From Pareto Point 1, the point with the highest probability of reaching the target, Pareto point 2 sacrifices only $1.9\%$ probability of target, but uses half the energy. However, while Pareto Point 3 represents another halving of the energy, the probability of target drops by $11.5\%$. Also note the stark comparison with the full KF performance; at its highest probability of reaching the target, ET achieves the similar performance for $54\%$ the energy use. 

% The behaviors of the three Pareto Points can be seen in the simulation of their corresponding strategies in Figure \ref{TrajectoryComp}.
Figure \ref{TrajectoryComp} shows 3000
% \ml{300 or 3000?}
simulated runs of each strategy, with the triggering threshold indicated by the color of the trajectory. Each threshold can be directly mapped to an expected triggering rate (see \cite{Wu2013}). The efficiency of the strategies can be seen in how the triggering rate only increases (lower $\delta$'s), contracting the trajectory, in proximity to obstacles. Trivially, we can see that the lower energy Pareto points correspond to lower triggering rates (higher $\delta$'s) around the obstacles. 

\begin{comment}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Set54ParetoFront.pdf}
         \caption{Pareto Front}
         \label{openPfront}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220307set54mergedMDPpp2.pdf}
         \caption{Pareto Point 1}
         \label{openPP1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{20220307set54mergedMDPpp6.pdf}
         \caption{Pareto Point 2}
         \label{openPP2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.07\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/colorbar.pdf}
     \end{subfigure}
        \caption{Pareto front and 2 simulated strategies for 2D System, open trajectory, using discretized belief method.}
        \label{openTrajectory}
\end{figure}

\at{I'm cutting this section to get it under 8 pages, capiche?}

The Pareto front is specific to the trajectory chosen. To demonstrate this, we consider a more open trajectory for the same 2D system with the Discretized Belief Method. This trajectory does not collide with any obstacles. The resulting Pareto Front and trajectories for two simulated points are shown in Figure \ref{openTrajectory}. Performance of the objectives for the two simulated Pareto points is shown in Table \ref{tab:2Dopen}.
\begin{table}[h!]
\begin{center}
    \caption{Two Pareto Points for open trajectory with Discretized Belief Method}
    \label{tab:2Dopen}
    \begin{tabular}{|| c | c | c | c ||}
    \hline
    Pareto Point & $P_{tar}$ & $P_{col}$ & $E_c$ \\
    \hline
         1 & 97.66\% & 0.0 & 52.58 \\
         2 & 95\% & 0.0 & 30.95\\
         Full KF & 97.43\% & 0.0 & 332.82\\
    \hline
    \end{tabular}
\end{center}
\end{table}

Note that because this trajectory avoids proximity with obstacles, the only difference in the Pareto Points comes at the very end of the trajectory going into the target region. Because there is really only one waypoint with a relevant action choice, the trade-offs between Pareto points are far less dramatic than the first trajectory, however the contrast with a using a full KF at every time step is amplified.

\end{comment}


\paragraph*{3D System}
Finally, to demonstrate the flexibility of our abstraction method, we consider the same system as (\ref{eq:2Ddynamics}), but extended to three dimensions. A selection of interesting Pareto Points and a single simulated strategy for a winding trajectory using the Discretized Belief Method is shown in Figure \ref{3DTrajectory}. Note that the same general shape of the Pareto front holds for the 3D system, with generous trade-offs at higher energies that taper as the energy decreases. The simulated trajectory corresponds to the highest probability of target and shows similar behavior to the 2D system, with higher triggering rates closer to the obstacles.
\vspace{-2mm}
\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Set53ParetoFront.pdf}
         \caption{Pareto Front}
         \label{3DPfront}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.235\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/20220307set53mergedMDPpp2View5-rotated.pdf}
         \caption{Pareto Point 1}
         \label{3DPP1}
     \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.07\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/colorbar.pdf}
    % \end{subfigure}

        \caption{(a) Pareto front and simulated strategy for 3D System; (b) `Super G' trajectory, using discretized belief method. } 
        \label{3DTrajectory}
        \vspace{-2mm}
\end{figure}

% evaluation.tex

==> sections/intro.tex <==
% intro.tex

As autonomous agents become more prevalent in society, it is increasingly important to find ways to efficiently and effectively deploy them. These systems must be able to reliably perform given tasks with limited resources. This is a difficult challenge given that these two aspects are naturally competing: often the best performance of a task comes at a greater expense of resources. One facet of this problem is the cost of accurate estimation of the system state; more measurements of the state leads to better estimation and hence better decisions, but this comes at some resource expense. This is a particularly troublesome issue for networked systems that rely on shared information, where communication cost competes with the accuracy of state estimation. 

For example, a system might combine mobile agents with remote sensors (Figure \ref{fig:EstimationDiagram}). While the sensors can make and communicate measurements with the agents, they may have limited computing capabilities and battery life. When  Conserving resources in this scenario necessarily means limiting the consumption of power in the remote sensing network. Additionally, systems may be bandwidth limited, in which case limiting communication frees up space for other valuable information, e.g. science data in exploration missions. In this paper, we develop a formal framework to explore optimal trade-offs 
between communication cost and task performance. 

A popular method of managing communication costs is event-triggered (ET) estimation \cite{Trimpe2015, Ouimet2018, Shi2014, Wu2013}. In the ET framework, information is only communicated when it is deemed useful. This condition can take many forms \cite{Trimpe2015}, but a common choice is a threshold on the innovation of a measurement \cite{Ouimet2018, Shi2014, Wu2013}. By changing this threshold, we can change the frequency of communication. While this can be a powerful tool for trading-off energy usage with estimator accuracy, there are no methods for tuning this threshold to guarantee the  trade-off is optimal and accounts for task performance. 

% Typical studies of resource efficiency in autonomy focus on a single objective, for example solely minimizing energy consumption \cite{Ondruska2015}. 
Trade-off analysis techniques have been studied mostly in formal methods literature \cite{Etessami2007,Forejt2012, Hahn:QEST:2017, Hahn:TOMACS:2019}.  
% The focus there is on the theoretical framework and include quantiles and multi-objective methods.
% Multi-objective optimization is a more complex problem, and is less widely studied in this field, but a good overview can be found in \cite{Romanova2020}. 
% Multi-objective verification and control synthesis is rooted in formal methods \cite{Etessami2007,Forejt2012}. 
Given a set of quantitative objectives and system model, the goal of multi-objective analysis is to calculate the set of all optimal trade-offs between the objectives, called the \emph{Pareto front}.  Recent studies explore applications in robotics \cite{Romanova2020}, path planning \cite{lavin2015pareto,Lee2018}, multi-agent coordination \cite{Zhao2021,Ghrist2006,Cui2012}, 
% and localization module selection in mobile robots \cite{Lahijanian2018}.  
% The methods proposed here are most closely related to  \cite{Lahijanian2018}, where methods were developed for optimally scheduling operation of a sensing module. In that case, the decision was whether or not to turn on a high precision, high cost sensor. Similar to this work, those methods focused on a trade off between state estimation accuracy and task performance. Our work looks at sensor network's communication costs, rather than a single agent's sensing module.
and sensor scheduling \cite{Lahijanian2018}.
The latter specifically focuses on resource and performance objectives and develops a scheduling framework for the usage of a high precision, high cost sensor. Nevertheless, finding Pareto-optimal communication strategies between a sensor network and mobile agents with respect to multiples objectives remains an open problem.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/processDiagram.pdf}
    \vspace{-2mm}
    \caption{Diagram of triggering and estimation process}
    \label{fig:EstimationDiagram}
    \vspace{0mm}
\end{figure}

In this paper, we fill this gap by introducing a method of synthesizing strategies for setting ET thresholds to achieve optimal trade-offs between resource consumption and task performance. We specifically consider a scenario where a mobile agent has to reach a goal region while avoiding unsafe states (obstacles) by communicating with a resource-limited remote sensor network. 
Our approach is based on abstracting this system to a discrete Markov Decision Process (MDP). The abstraction involves a novel belief space discretization method  %technique of discretizing the belief space 
using the spectral decomposition of the estimated covariance. 
We show this abstraction method is more efficient than alternatives and also benefits from interpretability. 
Then, we leverage off-the-shelf tools (PRISM \cite{Kwiatkowska2011}, PRISM-games \cite{Kwiatkowska2013}) to obtain the Pareto front and synthesize ET strategies for individual points on the front.  We show the efficacy of the approach in several case studies.

In short, the contributions are: (i) the use of multi-objective analysis to synthesize ET threshold strategies with optimal resource-performance trade-off guarantees, (ii) a novel technique to discretize a Gaussian belief based on the spectral decomposition of its covariance matrix, (iii) a method of using this discretization to abstract the continuous space system to an MDP, and (iv) a set of case studies that illustrate the efficacy of the method.


% \begin{itemize}
%     \item Given an environment and linear system model with Gaussian process and measurement noise, we provide a technique to calculate the optimal tradeoffs between competing objectives and, given a specific tradeoff, generate the corresponding ET threshold policy.
%     \item We propose a novel technique to discretize a Gaussian belief based on the spectral decomposition of its covariance matrix
%     \item We provide a method of using this discretization to abstract the continuous space system to an MDP
% \end{itemize}



==> sections/introFinal.tex <==
% intro.tex

As autonomous agents become more prevalent in society, they must be able to reliably perform given tasks with limited resources. This is a difficult challenge given that these two aspects are naturally competing: often the best performance of a task comes at a greater expense of resources. One facet of this problem is the cost of accurate estimation of the system state; more measurements of the state can be costly, but lead to better estimation and hence better decisions. This is a particularly troublesome issue for networked systems that rely on shared information, where communication cost directly competes with the accuracy of state estimation. 

For example, a system might combine mobile agents with remote sensors as shown in Figure \ref{fig:EstimationDiagram}. While the sensors can make and communicate measurements with the agents, they may have limited computing capabilities and battery life and, in remote environments, may be difficult to access to change batteries. According to \cite{Shi2014:ML}, wireless transmission is at least an order of magnitude more costly in terms of energy consumption than any other function in a standard ZigBee networking chip. Maintaining consistent operation in these kinds of scenarios necessarily means limiting  communication in the remote sensing network. Additionally, systems may be bandwidth limited, in which case limiting communication frees up space for other valuable information, e.g., science data in robotic exploration missions. In this paper, we develop a formal framework to explore optimal trade-offs between communication cost and task performance. 

A popular method of managing communication costs is event-triggered (ET) estimation \cite{Trimpe2015, Ouimet2018, Shi2014, Wu2013}. In the ET framework, information is only communicated when it is deemed useful. This condition can take many forms \cite{Trimpe2015}, but a common choice is a threshold on the innovation of a measurement \cite{Ouimet2018, Shi2014, Wu2013}. Changing this threshold changes the frequency of communication. While this can be a powerful tool for resource-performance trade-off, there are no methods for tuning this threshold to guarantee the  trade-off is optimal and accounts for task performance. 

Trade-off analysis techniques have been studied mostly in formal methods literature \cite{Etessami2007,Forejt2012, Hahn:QEST:2017, Hahn:TOMACS:2019}. Given a set of quantitative objectives and system model, the goal of multi-objective analysis is to calculate the set of all optimal trade-offs between the objectives, called the \textit{Pareto front}.  Recent studies explore applications in robotics \cite{Romanova2020}, path planning \cite{lavin2015pareto,Lee2018}, multi-agent coordination \cite{Zhao2021,Ghrist2006,Cui2012}, and sensor scheduling \cite{Lahijanian2018}.
The latter specifically focuses on resource and performance objectives and develops a scheduling framework for the usage of a high precision, high cost sensor. Nevertheless, finding Pareto-optimal communication strategies between a sensor network and mobile agents with respect to multiple objectives remains an open problem.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/processDiagram.pdf}
    \vspace{-1mm}
    \caption{Diagram of triggering and estimation process.}
    \label{fig:EstimationDiagram}
    \vspace{-4mm}
\end{figure}

In this paper, we fill this gap by introducing a method of synthesizing strategies for setting ET thresholds to achieve optimal trade-offs between resource consumption and task performance. We specifically consider a scenario where a mobile agent has to reach a goal region while avoiding unsafe states (obstacles) by communicating with a resource-limited remote sensor network. 
Our approach is based on abstracting this system to a discrete Markov Decision Process (MDP). The abstraction involves a novel belief space discretization method using the spectral decomposition of the estimated covariance. 
We show this abstraction method is more efficient than alternatives and also benefits from interpretability. Then, we leverage off-the-shelf tools (PRISM \cite{Kwiatkowska2011}, PRISM-games \cite{Kwiatkowska2013}) to obtain the Pareto front and synthesize ET strategies for individual points on the front.  We show the efficacy of the approach in several case studies.

%In short, the contributions are: (i) the use of multi-objective analysis to synthesize ET threshold strategies with optimal resource-performance trade-off guarantees, (ii) a novel technique to discretize a Gaussian belief based on the spectral decomposition of its covariance matrix, (iii) a method of using this discretization to abstract the continuous space system to an MDP, and (iv) a set of case studies that illustrate the efficacy of the method.


==> sections/methodology.tex <==
% problem.tex

% Analysis on an MDP reasons over a discrete set of states, which means existing analysis methods cannot be directly applied to continuous space systems. 
Finite abstraction is often performed via a discretization of the continuous state space.
In absence of sensing uncertainty, this is easily addressed by polytopic partitions, e.g., a grid. However, with measurement noise, the true state of the system is unknown; hence, we must reason over the belief space. 
Recall from \eqref{eq:beldef} that the belief at a waypoint is dependent on the history of measurements and threshold choice. Consequently, the belief evolution captured at waypoints is as an exponentially growing graph \cite{Lahijanian2018}. 
To avoid such explosion, we seek discretization methods that break the history dependence.
Specifically, 
we achieve this by either enforcing convergence to a single belief at a waypoint or by grouping the beliefs at each waypoint.  Then, the transition from a belief $b$ at waypoint $\wp_i$
to another belief at $\wp_{i+1}$ 
becomes dependent only on $b$ and the choice $\delta$ at $\wp_i$, not on the entire history. This naturally leads to an MDP construction where the MDP states are formed by the converged belief or belief sets.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/BeliefGraph.pdf}
%     \caption{Exponentially growing belief, red arrows indicate no trigger occurred, green arrows indicate trigger did occur.}
%     \label{fig:beliefGraph}
%     \vspace{0mm}
% \end{figure}

Existing methods, like \cite{AghaMohammadi2014} and \cite{Lahijanian2018}, rely on convergence to a known belief. Our first proposed method is an arguably trivial extension of this existing work, wherein we enforce convergence to steady state beliefs about the waypoints. However, we demonstrate that this naive approach yields too coarse a gradation in the Pareto front, and does not fully reap the energy savings offered by ET. To address this, we develop a novel abstraction method that exploits the inherent geometry of the variable covariance hyperellipsoids obtained under ET to discretize and group similar beliefs together.




%% MDP Definition %%
\subsection{MDP Abstraction}
An MDP $\mathcal{M}=(S, s_0, A, T, \costMDP)$ is a tuple consisting of a finite set of states $S$, an initial state $s_0 \in S$, a set of actions $A$, a probabilistic transition function $T: S \times A \rightarrow [0,1]$, and a cost function $\costMDP: S \times A \rightarrow \mathbb{R}_{\geq0}$ that assigns to each state-action pair to a non-negative cost.

In our MDP abstraction, the action set $A = \Delta$, the set of ET thresholds, and each state $s \in S$ is defined as a set of beliefs at each waypoint. %The formulation of these sets is defined in the following sections. 
The cost $\costMDP(s,\delta)$, where $\delta \in \Delta$, is the expected communication cost from the waypoint $\wp$ corresponding to MDP state $s$, to the next waypoint, and is given by
\begin{equation}
    \costMDP(s,\delta) = \bar{k}(\wp,\delta) \, \gamma(\delta),
\end{equation}
where $\bar{k}(\wp,\delta)$ is the expected number of time steps required to navigate from $\wp$ to the the next waypoints under $\delta$. 
Further, we include three states $s_\coll$, $s_\tar$, and $s_{\mathrm{free}}$ in addition to the belief states in $S$ to represent termination in an obstacle, target region, and neither, respectively. %obstacle nor target.

Below, we detail two methods to construct the MDP states: enforced KF convergence and discretized belief states.
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/BeliefConvergeMethod.pdf}
    \caption{Diagram of Belief Convergence method}
    \label{fig:beliefConvergence}
    \vspace{0mm}
\end{figure}

\begin{figure*}
    \centering
    \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{CovEllipse.pdf}
    \caption{}
    %\caption{Example 2D covariance ellipse decomposed via eigenvalues $\lambda_i$ and eigenvectors $v_i$.}
    \label{fig:covEll}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/DiscEllipse1.pdf}
    \caption{}
    %\caption{Angle discretization of a single axis, with the nominal vector shown as a red dashed line}
    \label{fig:DiscEllAngles}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figures/DiscEllipse2.pdf}
    \caption{}
    %\caption{Magnitude discretization of a single axis, with the nominal vector shown as a red dashed line}
    \label{fig:DiscEllMagnitudes}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figures/DiscEllipse3.pdf}
    \caption{}
    %\caption{Full Region discretization of a single axis, with the nominal vector shown as a red dashed line}
    \label{fig:DiscEllRegions}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.19\textwidth}
    \includegraphics[width=\textwidth]{figures/DiscEllipse4.pdf}
    \caption{}
    %\caption{Sample covariance contained within a state defined by a region in the first axis (shown in red and discretized as in c.), and a region in the second axis (shown in blue).}
    \label{fig:DiscEllTest}
    \end{subfigure}
\caption{(a) Example 2D covariance ellipse decomposed via eigenvalues $\lambda_i$ and eigenvectors $v_i$. (b) Magnitude discretization of a single axis, with $v_{nom}$ shown as a red dashed line.  (c) Angle discretization of a single axis, with $v_{nom}$ shown as a red dashed line.  (d) Full region discretization of a single axis. %, with the nominal vector shown as a red dashed line. 
(e) Sample covariance contained within a state defined by a region in the first axis (shown in red and discretized as in c.), and a region in the second axis (shown in blue).}


%\vspace{0mm}
\end{figure*}
%% Method 1
\subsection{Method 1: Enforced Belief Convergence} 

This method relies on convergence to a pre-computed belief to break the history dependence of the belief graph discussed above.
% shown in Figure \ref{fig:beliefGraph}. 
% Because the belief converges to a known distribution at each waypoint, the transition from one waypoint to another becomes independent of the history from prior waypoints. 
This pre-computed belief at waypoint $\wp$ is a Gaussian distribution defined by the KF steady state covariance $P_\text{KF} \in \mathbb{R}^{n \times n}$, i.e., $\mathcal{N}(\wp, P_\text{KF})$.
% the mean convergence criteria in \eqref{eq:meanConvCond}. %%Thus, the belief state at each waypoint (MDP state $s$) is known to be Gaussian with covariance within some tolerance of $P_{KF}$ and mean within some tolerance of the waypoint.


To ensure convergence to this belief, we force the system to switch from ET to KF estimation within some neighborhood of $\wp$. 
Let $\tol_\text{KF}\in\mathbb{R}_{>0}$ be the radius of this neighborhood.   
% around each waypoint within which we switch from ET to a basic KF (where all measurements are communicated). Define the estimation mode as $\mathcal{M}_k \in \{0,1\}$, where $\mathcal{M}_k=1$ indicates estimation via ET, and $\mathcal{M}=0$ indicates estimation via KF. When the system initially begins its traverse to the next waypoint, the initial mode is set to $\mathcal{M}=1$. It then travels toward the next waypoint until the switching condition is met and the estimator changes to $\mathcal{M}=0$:
% \begin{equation}
%     \|\hat{x}_k - \wp_{i+1}\|_2 \leq \tol_{KF} \rightarrow  \mathcal{M}_{k+1}=0.
% \end{equation}
% The system then continues in mode $\mathcal{M}=0$ until the previously defined convergence criteria in \eqref{eq:meanConvCond} is met, \emph{in addition to} covariance convergence criterion, defined as 
% \begin{equation}
% \label{eq:covConvCond}
%     \|P_k - P_{KF}\|_{max} \leq \tol_P,
% \end{equation}
% where  $P_k$ is the covariance at time $k$, $\tol_P \in \mathbb{R}_{>0}$ is the tolerance, and the max-norm, $\|\cdot\|_{max}$, indicates the maximum element of a matrix. 
The system switches to KF when $\|\hat{x}_k - \wp_{i+1}\|_2 \leq \tol_{KF}$.  Then, it continues under KF until both the covariance convergence condition, $\|P_k - P_{KF}\|_{max} \leq \tol_P$, where $\tol_P \in \mathbb{R}_{>0}$, and \eqref{eq:meanConvCond}, are met.  
See Figure \ref{fig:beliefConvergence} for reference.
The belief state at each waypoint is thus known to be Gaussian with a covariance within $\tol_P$ of $P_{KF}$ and a mean within $\tol_x$ of the waypoint. So, the MDP state under the Enforced KF Convergence Method is defined as a tuple: 
$s = (\wp, \tol_x, P_{KF}, \tol_P).$
% , where $\wp$ is the waypoint, $\tol_x$ is the tolerance defining convergence of the state to the waypoint (see \eqref{eq:meanConvCond}), $P_{KF}$ is the KF steady state covariance, and $\tol_P$ is the tolerance defining convergence of the covariance to $P_{KF}$ (see \eqref{eq:covConvCond}). 

Note that, under every choice of $\delta$,  the system converges to the same MDP belief state at each waypoint. Hence, one of the benefits of this method is its low complexity: the total number of states is $N+3$, where $N$ is the number of waypoints.  It however suffers from constraining the system and does not fully exploit the benefits of ET estimation.

%% Method 2
\subsection{Method 2: Discretized Belief State}
The second method operates only in the ET mode
% , $\mathcal{M}_k=1$, $\forall k$, 
and uses only the mean convergence criterion in \eqref{eq:meanConvCond} for termination. %No further convergence criteria is enforced on the covariance. 
This means $P_k$ at each waypoint can be quite variable. As there are two possible cases for the $P_k$ update (implicit and explicit information updates), stochastic $y_k$ induces random switching between these two cases. This switching precludes convergence to steady state $P_k$; even under the same $\delta$, two trajectories may arrive at the same waypoint with drastically different $P_k$. 
We form the MDP states from sets of $b_k$ at each waypoint with $\hat{x}_k$ captured by criterion in \eqref{eq:meanConvCond} and $P_k$ captured by a discretized covariance state (described below). The obtained MDP using this grouping of beliefs leads to history-independent state transitions only up to the resolution used for the covariance discretization, called \textit{abstraction error}.
% In practice, history dependence is still present if the discretization step size is large. 
In Sec. \ref{subsec:DiscErr}, we show that the abstraction error goes to zero as the discretization size goes to zero.

\begin{comment}

\ml{what is the high-level idea? What are the key observations? Based on the key ideas and observations, define the method.} \at{I tried to lay out the key observations and intuition in the intro to this section, it just seemed to fit better} \na{concur with Morteza -- the text and figure for the geometric intuition part should go here and a much more succinct/shorter statement describing the second approach should be given at the top/intro of the section.}

If the convergence condition on the belief is relaxed, the mean of the belief still converges (under \eqref{eq:meanConvCond}), but the the covariance does not. This is due to the nature of the implicit vs explicit information update in ET estimation: explicit information reduces uncertainty, while implicit information inflates uncertainty \na{need to sharpen this statement, since it's not precise and easy to misinterpret -- the whole point of having/using the implicit information is to keep the uncertainty from exploding in the state estimator (otherwise it's not information/informative at all!) -- covariance will be reduced less with implicit info than explicit info, but it is not the same as inflating/increasing uncertainty, through say naive pure filter prediction with no measurement updates at all}. The stochasticity of the measurements induces random switching between implicit and explicit updates, and consequentially a continuous range over the covariance matrices at each waypoint. Different covariances correspond to different beliefs at the waypoints. We form a discrete model by grouping the beliefs into discrete sets, then using these sets as MDP states. 
\end{comment}

The simplest approach is to directly discretize the individual elements of $P_k$. However, this approach is inefficient and exacerbates the state explosion problem. Instead, we rely on a geometric interpretation of $P_k$: 
the spectral decomposition of $P_k$ results in $n$ eigenvectors and eigenvalues, which respectively describe the orientation axes and magnitudes of an associated uncertainty (hyper)ellipse, as shown in Figure \ref{fig:covEll}. 
%We define a \emph{region} for each of these $n$ axes. 
The covariance state is then taken as a combination of discrete \emph{regions} across each axis. %, describing the angle and orientation of each axis of the covariance ellipse. 
%The eigenvectors of the decomposition describe the orientation of the axes of the ellipse, and the eigenvalues their magnitude. This geometric interpretation naturally extends to a geometric discretization based on axis magnitudes and angles. 


%Thus, the new method described here implements a geometric discretization to directly discretize the belief space. 
%The spectral decomposition of the covariance matrix results in $n$ eigenvectors and their associated $n$ eigenvalues. We define a \emph{region} for each of these $n$ dimensions, or axes. The covariance state is taken as a combination of regions across each axis (describing the angle and orientation of each axis of the covariance ellipse). 

A discrete region for each axis (eigenvector) is defined by 3 elements: a nominal vector, an angle range, and a magnitude range. The nominal vector, $v_{nom} \in \mathbb{R}^n$, is a unit vector that provides the orientation of the region. While the nominal vector can be chosen as any vector in $\mathbb{R}^n$, a good choice is to base it on empirically sampled data. The angle range between $\theta_{low}, \theta_{high} \in (0,\pi/2]$, is defined \emph{relative} to the $v_{nom}$, with the angle calculated via the Euclidean inner product, (various angle choices are shown in \ref{fig:DiscEllAngles}). The magnitude range is between $\lambda_{low}, \lambda_{high} \in \reals_{>0}$ (various magnitude choices are shown in Figure \ref{fig:DiscEllMagnitudes}). A region described by $v_{nom}$, angles $\theta_{low}$ and $\theta_{high}$, and magnitudes $\lambda_{low}$ and $\lambda_{high}$, is defined as the set %of angles and magnitudes:
\begin{equation}
    R = \{(\lambda, \theta) \mid \lambda \in [\lambda_{low}, \lambda_{high}) \wedge \theta \in [\theta_{low}, \theta_{high})\},
\end{equation}
for eigenvalue $\lambda$ and angle $\theta$ from the eigenvector to $v_{nom}$ (the combinations of angle and magnitude ranges to form
regions are shown as colored areas in Figure \ref{fig:DiscEllRegions}).
%A pictorial reference is provided in Figure \ref{discEll}. %%: in \ref{discEll}.a-c, the nominal vector is shown as a red dashed line, \ref{discEll}.a. shows various magnitude ranges, and \ref{discEll}.b. shows various angle ranges. The combination of all three elements defines the regions, shown as filled areas in \ref{discEll}.c.. 

The full covariance state, $c_R$ is taken as a combination of regions for each dimension: $c_R = (R_1, ..., R_n)$. Figure \ref{fig:DiscEllTest} shows the decomposition of an example covariance, and the covariance state it falls in. The MDP state under the Discretized Belief State Method is defined as a tuple: $s = (\wp, \tol_x, c_R)$.

Defining the states as described relies on some knowledge of the upper and lower bounds of the covariance. While the lower bound can be trivially obtained via the KF steady state covariance, we currently have no method of determining the theoretical upper bound for the covariance. Although this is a potential avenue for future work, a good empirical bound can be obtained by propagating the covariance through the update equation and enforcing $\gamma_k=0$ at every time step. 
\begin{comment}
% where $\wp$ is the waypoint, $\tol_x$, is the tolerance defining convergence of the state to the waypoint (see \eqref{eq:meanConvCond}), and $s_R$ is the covariance state. 
\ml{didn't we just cover this above?}
The covariance state is defined in as a tuple of the component regions: $c_R = (R_1, ..., R_n)$. Each region is a tuple containing the nominal vector, angle range, and magnitude range: $R_i=(v_{nom,i}, \Theta_i, \Lambda_i)$, where each $\Lambda_i$, $i=1,..,n$, defines a low and high pair of magnitudes for each axis ($(\lambda_{low},\lambda_{high}) \in \mathbb{R}_{>0}$), each $\Theta_i$, $i=1,..,n$, defines a low and high pair of angles for each axis ($(\theta_{low},\theta_{high})  \in (0,\pi/2]$), and each $v_{nom,i} \in \mathbb{R}^n$, $i=1,..,n$, defines a nominal vector for each axis. \na{from the `A discrete region for each axis...' paragraph on: feels repetitive and over-explained, should be sharper and more succinct/to the point (and more precise, per ML's comments above). Let the math and Fig. 4 do the talking, only spend extra words to explain things that are not intuitive/obvious.}

\end{comment}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{DiscEllipse.pdf}
%     \caption{a.-c.) show the discretization of a single axis, with the nominal vector shown as a red dashed line. a.) shows various magnitude ranges, b.) shows various angle ranges, and c.) shows the combinations of these to form discrete regions, each shown as a colored area. d.) shows a sample covariance contained within a state defined by a region in the first axis (shown in red and discretized as in c.), and a region in the second axis (shown in blue).
%     \ml{fix the axes...}
%     }
%     \label{discEll}
%     \vspace{0mm}
% \end{figure}

\subsubsection{Discretization Error}
\label{subsec:DiscErr}
Modeling errors arise whenever a continuous state space dynamical system is spatially discretized. In the MDP, this error presents in the transition probabilities: belief states originating from some parts of the same region (as defined above) have different transition probabilities from those originating in different parts of the same region. This discrepancy in the probabilities is the abstraction error. Theorem \ref{theorem}  shows that as the volume of the discretized belief state, i.e. the size of the ranges $(\theta_{low}, \theta_{high})$ and $(\lambda_{low}, \lambda_{high})$, goes to zero, the abstraction error goes to zero.

\begin{theorem}\label{theorem}
Consider the transition from a set of belief states $\mathcal{S}$ to another set $\mathcal{S}'$. The volume of each set is defined by the discretization sizes: $d\lambda=\lambda_{high}-\lambda_{low}$, $d\theta=\theta_{high}-\theta_{low}$. Assume $d\lambda$ and $d\theta$ are equivalent for $\mathcal{S}$ and $\mathcal{S}'$. Every point in the originating set, $s \in \mathcal{S}$, has an associated transition probability to $\mathcal{S}'$, $P(\mathcal{S}'|s)$. The maximum difference between transition probabilities within the set is:
\begin{equation}
    \Delta P_{max}=\max_{s_1,s_2\in \mathcal{S}} |P(\mathcal{S}'|s_1) - P(\mathcal{S}'|s_2)|.
\end{equation}
As the discretization step sizes go to zero, this difference must also go to zero:
\begin{equation}
    \lim_{d\lambda \to 0, d\theta\to 0} \Delta P_{max} = 0.
\end{equation}

\end{theorem}

\begin{proof}

Within the set $\mathcal{S}$, there must exist some point, $s_{max}$, that maximizes the transition probability, and some point, $s_{min}$, that minimizes this probability:
\begin{equation}
    s_{max}=\max_{s\in \mathcal{S}} P(\mathcal{S}'|s), \quad s_{min}=\min_{s\in \mathcal{S}} P(\mathcal{S}'|s).
\end{equation}

Now, consider a new set that is strictly a subset of $\mathcal{S}$, $\tilde{\mathcal{S}}\subset \mathcal{S}$. Because it is a subset of $\mathcal{S}$, we can use $\tilde{\mathcal{S}}$ to bound the probabilities:
\begin{align}
\max_{s\in \mathcal{S}} P(\mathcal{S}'|s) \leq \max_{s\in \tilde{\mathcal{S}}} P(\mathcal{S}'|s) \\
\min_{s\in \mathcal{S}} P(\mathcal{S}'|s) \geq \min_{s\in \tilde{\mathcal{S}}} P(\mathcal{S}'|s).
\end{align}
In the limit as the volume of $\mathcal{S}$ goes to zero, these bounds must converge to each other. Thus, the difference in probabilities within the volume, $\Delta P_{max}$,  must also go to zero.
\end{proof}

\subsubsection{Scalability}
A simpler method of covariance discretization could involve setting ranges on the individual elements of the covariance matrix, rather than relying on the spectral decomposition. While attractive in its simplicity, this alternative exacerbates an existing problem with discretization: state explosion. Consider an analogous definition of a region as some range of values over a single element of the covariance matrix. The full MDP state could then be described as a combination of regions across each element of the covariance matrix. Since the covariance matrix is symmetric, the number of regions, $N_R$, required to describe a state is
\begin{equation}
    N_R = \frac{n(n+1)}{2},
\end{equation}
where $n$ is the dimension of the state space. Whereas the spectral decomposition requires only a single region for each axis, so the number of regions required to describe a state is simply $n$.

Now assume that each matrix element is discretized into $d$ regions, and similarly that each axis in the spectral decomposition is also discretized into $d$ regions. The total number of combinations across all the regions is $d^{N_R}$. While this number explodes for both cases, it explodes less rapidly for the discretization based on the spectral decomposition. If we assume the same discretization at every waypoint, the total number of states is then $Nd^{N_R}+3$. While this is a worst case scenario (in practice, not every combination of regions is occupied), the described techniques do suffer from a state explosion problem, which is particularly troublesome as the dimensionality of the system increases.

The number of required regions for the matrix elements could be reduced by adding constraints inherent to the covariance, like positive definiteness and orthogonality. However, interpreting these constraints in matrix form is not straightforward, while they are very simple to implement in a spectral decomposition. The spectral decomposition also benefits from visual interpretability; it is easy to visualize the uncertainty of the system in terms of vectors defining a covariance ellipse. 

Off the shelf tools are available to solve the multi-objective problem on an MDP \cite{Kwiatkowska2011}. These use value iteration to construct a Pareto Front \cite{Forejt2012}, from which specific strategies are generated through linear programming \cite{Etessami2007}. The MDP analysis algorithms are polynomial with the size of the MDP.

For both methods, we use Monte Carlo sampling to approximate the transition probabilities \cite{Lahijanian2018}.


==> sections/methodologyFinal.tex <==
% problem.tex

% Analysis on an MDP reasons over a discrete set of states, which means existing analysis methods cannot be directly applied to continuous space systems. 
Finite abstraction is often performed via a discretization of the continuous state space. In absence of sensing uncertainty, this is easily addressed by polytopic partitions, e.g., a grid. However, with measurement noise, the true state of the system is unknown; hence, we must reason over the belief space. Recall from \eqref{eq:beldef} that the belief at a waypoint is dependent on the complete history of measurements and threshold choices. Consequently, the belief evolution is an exponentially growing graph \cite{Lahijanian2018}. To avoid analysis of the full graph, we propose two abstraction methods via (i) enforcing convergence to a single belief at each waypoint, and (ii) grouping the beliefs at each waypoint (analogous to a polytopic discretization of state space). With these methods, the transition from a belief $b$ at waypoint $\wp_i$ to another belief at $\wp_{i+1}$ becomes dependent only on $b$ and the choice $\delta$ at $\wp_i$. This naturally leads to an MDP abstraction where the MDP states are formed by the converged belief or belief sets.

% Existing methods, like \cite{AghaMohammadi2014} and \cite{Lahijanian2018}, rely on convergence to a known belief. Our first proposed method is an arguably trivial extension of those existing works. However, we demonstrate that this naive approach does not fully reap the energy savings offered by ET. Our second method addresses this issue by using a novel abstraction method that exploits the inherent geometry of the covariance hyperellipsoids to discretize by grouping similar beliefs together.

\begin{figure*}
    \centering
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[width=\textwidth]{CovEllipse.pdf}
        \vspace{-7mm}
        \caption{}
        %\caption{Example 2D covariance ellipse decomposed via eigenvalues $\lambda_i$ and eigenvectors $v_i$.}
        \label{fig:covEll}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/DiscEllipse1.pdf}
        \vspace{-7mm}
        \caption{}
        %\caption{Angle discretization of a single axis, with the nominal vector shown as a red dashed line}
        \label{fig:DiscEllAngles}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/DiscEllipse2.pdf}
        \vspace{-7mm}
        \caption{}
        %\caption{Magnitude discretization of a single axis, with the nominal vector shown as a red dashed line}
        \label{fig:DiscEllMagnitudes}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/DiscEllipse3.pdf}
        \vspace{-7mm}
        \caption{}
        %\caption{Full Region discretization of a single axis, with the nominal vector shown as a red dashed line}
        \label{fig:DiscEllRegions}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.18\textwidth}
        \includegraphics[width=\textwidth]{figures/DiscEllipse4.pdf}
        \vspace{-7mm}
        \caption{}
        %\caption{Sample covariance contained within a state defined by a region in the first axis (shown in red and discretized as in c.), and a region in the second axis (shown in blue).}
        \label{fig:DiscEllTest}
    \end{subfigure}
\caption{(a) Example 2D covariance ellipse decomposed via eigenvalues $\lambda_i$ and eigenvectors $v_i$. (b) Magnitude discretization of a single axis, with $v_{nom}$ shown as a red dashed line.  (c) Angle discretization of a single axis, with $v_{nom}$ shown as a red dashed line.  (d) Full region discretization of a single axis. %, with the nominal vector shown as a red dashed line. 
(e) Sample covariance contained within a state defined by a region in the first axis (shown in red and discretized as in c), and a region in the second axis (shown in blue).}
\vspace{-3mm}
\end{figure*}


%% MDP Definition %%
\subsection{MDP Abstraction}
An MDP $\mathcal{M}=(S, s_0, A, T, \costMDP)$ is a tuple consisting of a finite set of states $S$, an initial state $s_0 \in S$, a set of actions $A$, a probabilistic transition function $T: S \times A \rightarrow [0,1]$, and a cost function $\costMDP: S \times A \rightarrow \mathbb{R}_{\geq0}$ that assigns to each state-action pair to a non-negative cost.

In our MDP abstraction, each state $s \in S$ is defined as a set of beliefs at each waypoint, and the action set is the set of ET thresholds, i.e., $A = \Delta$. %The formulation of these sets is defined in the following sections. 
The cost $\costMDP(s,\delta)$, where $\delta \in \Delta$, is the expected communication cost from the waypoint $\wp$ corresponding to $s$, to the next waypoint, and is given by
\begin{equation}
    \costMDP(s,\delta) = \bar{k}(\wp,\delta) \, \gamma(\delta),
\end{equation}
where $\bar{k}(\wp,\delta)$ is the expected number of time steps required to navigate from $\wp$ to the the next waypoints under $\delta$. 
Further, we include three states $s_\coll$, $s_\tar$, and $s_{\mathrm{free}}$ in addition to the belief states in $S$ to represent termination in an obstacle, target region, and neither, respectively. %obstacle nor target.

Below, we detail two methods to construct the MDP states: enforced KF convergence and discretized belief states. For both methods, we use Monte Carlo sampling to approximate the transition probabilities, $T$ \cite{Lahijanian2018}.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/BeliefConvergeMethod.pdf}
%     \caption{Diagram of Belief Convergence method}
%     \label{fig:beliefConvergence}
%     \vspace{0mm}
% \end{figure}



%% Method 1
\subsection{Method 1: Enforced Belief Convergence} 

This method relies on convergence to a pre-computed Gaussian belief at waypoint $\wp$, and is defined by the KF steady state covariance $P_\text{KF} \in \mathbb{R}^{n \times n}$, i.e., $\mathcal{N}(\wp, P_\text{KF})$.


To ensure convergence to this belief, we force the system to switch from ET to KF estimation within some neighborhood of $\wp$. Let $\tol_\text{KF}\in\mathbb{R}_{>0}$ be the radius of this neighborhood. The system switches to KF when $\|\hat{x}_k - \wp_{i+1}\|_2 \leq \tol_{KF}$.  Then, it continues under KF until both the covariance convergence condition, $\|P_k - P_{KF}\|_{max} \leq \tol_P$, where $\tol_P \in \mathbb{R}_{>0}$, and \eqref{eq:meanConvCond}, are met.  
% See Figure \ref{fig:beliefConvergence} for reference.
The belief state at each waypoint is thus known to be Gaussian with a covariance within $\tol_P$ of $P_{KF}$ and a mean within $\tol_x$ of the waypoint. So, the MDP state under the Enforced KF Convergence Method is defined as a tuple: 
$s = (\wp, \tol_x, P_{KF}, \tol_P).$

Note that, under every choice of $\delta$,  the system converges to the same MDP belief state at each waypoint, hence the total number of states is $N+3$, where $N$ is the number of waypoints. Despite its low complexity, this method suffers from overly constraining the system, and thus does not fully exploit the benefits of ET estimation.

%% Method 2
\subsection{Method 2: Discretized Belief State}
The second method operates only in the ET mode and uses only the mean convergence criterion in \eqref{eq:meanConvCond} for termination. Stochastic $y_k$ induces random switching between the two possible cases for the $P_k$ information update (implicit and explicit), precluding convergence to steady state $P_k$. This means $P_k$ at each waypoint can be quite variable. Therefore, we form the MDP states from sets of $b_k$ at each waypoint with $\hat{x}_k$ captured by criterion in \eqref{eq:meanConvCond} and $P_k$ captured by a discretized covariance state (described below). The MDP obtained using this technique leads to history-independent state transitions only up to the resolution used for the covariance discretization, called \textit{abstraction error}. In the full version of this work \cite{Theurkauf2022}, we show that the abstraction error goes to zero as the discretization size goes to zero.

\begin{comment}

\ml{what is the high-level idea? What are the key observations? Based on the key ideas and observations, define the method.} \at{I tried to lay out the key observations and intuition in the intro to this section, it just seemed to fit better} \na{concur with Morteza -- the text and figure for the geometric intuition part should go here and a much more succinct/shorter statement describing the second approach should be given at the top/intro of the section.}

If the convergence condition on the belief is relaxed, the mean of the belief still converges (under \eqref{eq:meanConvCond}), but the the covariance does not. This is due to the nature of the implicit vs explicit information update in ET estimation: explicit information reduces uncertainty, while implicit information inflates uncertainty \na{need to sharpen this statement, since it's not precise and easy to misinterpret -- the whole point of having/using the implicit information is to keep the uncertainty from exploding in the state estimator (otherwise it's not information/informative at all!) -- covariance will be reduced less with implicit info than explicit info, but it is not the same as inflating/increasing uncertainty, through say naive pure filter prediction with no measurement updates at all}. The stochasticity of the measurements induces random switching between implicit and explicit updates, and consequentially a continuous range over the covariance matrices at each waypoint. Different covariances correspond to different beliefs at the waypoints. We form a discrete model by grouping the beliefs into discrete sets, then using these sets as MDP states. 
\end{comment}

A naive approach would be to directly discretize the individual elements of the $P_k$ matrix. However, as we show later, this approach is inefficient and exacerbates the state explosion problem. Instead, we rely on the spectral decoposition of $P_k$, which  results in $n$ eigenvectors describing the orientation of the axes and $n$ eigenvalues describing the magnitudes of an associated uncertainty (hyper)ellipse, as shown in Figure \ref{fig:covEll}. The covariance state is then taken as a combination of discrete \emph{regions} across each of the $n$ axes. 

A discrete region for each axis is defined by 3 elements: a nominal vector, an angle range, and a magnitude range. The nominal vector, $v_{nom} \in \mathbb{R}^n$, is a unit vector that provides the orientation of the region. While the nominal vector can be chosen as any vector in $\mathbb{R}^n$, a good choice is to base it on empirically sampled data. The angle range between $\theta_{low}, \theta_{high} \in (0,\pi/2]$, is defined \emph{relative} to the $v_{nom}$, with the angle calculated via the Euclidean inner product. The magnitude range is between $\lambda_{low}, \lambda_{high} \in \reals_{>0}$. Various angle and magnitude choices are shown in Figures \ref{fig:DiscEllAngles} and \ref{fig:DiscEllMagnitudes}. A region described by $v_{nom}$, angles $\theta_{low}$ and $\theta_{high}$, and magnitudes $\lambda_{low}$ and $\lambda_{high}$, is defined as the set
\begin{equation}
    R = \{(\lambda, \theta) \mid \lambda \in [\lambda_{low}, \lambda_{high}) \wedge \theta \in [\theta_{low}, \theta_{high})\},
\end{equation}
for eigenvalue $\lambda$ and angle $\theta$ from the eigenvector to $v_{nom}$ (the combinations of angle and magnitude ranges to form 
regions are shown as colored areas in Figure \ref{fig:DiscEllRegions}).
%A pictorial reference is provided in Figure \ref{discEll}. %%: in \ref{discEll}.a-c, the nominal vector is shown as a red dashed line, \ref{discEll}.a. shows various magnitude ranges, and \ref{discEll}.b. shows various angle ranges. The combination of all three elements defines the regions, shown as filled areas in \ref{discEll}.c.. 

The full covariance state, $c_R$ is taken as a combination of regions for each dimension: $c_R = (R_1, ..., R_n)$. Figure \ref{fig:DiscEllTest} shows the decomposition of an example covariance, and the corresponding $c_R$ it falls in. 
The MDP state under the Discretized Belief State Method is defined as a tuple: $s = (\wp, \tol_x, c_R).$

Defining the states as described relies on some knowledge of the upper and lower bounds of the covariance. While the lower bound can be trivially obtained via the KF steady state covariance, we currently have no method of determining the theoretical upper bound for the covariance. Although this is a potential avenue for future work, a good empirical bound can be obtained by propagating the covariance through the update equation and enforcing $\gamma_k=0$ at every time step. Additionally, the angle and magnitude ranges are also empirically chosen such that the abstraction error (discuss in the following section) is low, but the number of samples required for Monte Carlo sampling is not too large.

\subsubsection{Discretization Error}
\label{subsec:DiscErr}
Abstraction errors due to discretization manifest
in the transition probabilities: belief states originating from some parts of the same region (as defined above) have different transition probabilities from those originating in different parts of the same region. 
We provide a proof in the full version of this work \cite{Theurkauf2022} that as the volume of the discretized belief state, i.e., the size of the ranges $(\theta_{low}, \theta_{high})$ and $(\lambda_{low}, \lambda_{high})$, goes to zero, the abstraction error goes to zero.
% This discrepancy in the probabilities is the abstraction error. 
% Theorem \ref{theorem}  shows that as the volume of the discretized belief state, i.e., the size of the ranges $(\theta_{low}, \theta_{high})$ and $(\lambda_{low}, \lambda_{high})$, goes to zero, the abstraction error goes to zero.

% \begin{theorem}\label{theorem}
%     \ml{fix the statement of the theorem}
%     Consider the transition from a set of belief states $\mathcal{S}$ to another set $\mathcal{S}'$. The volume of each set is defined by the discretization sizes: $d\lambda=\lambda_{high}-\lambda_{low}$, $d\theta=\theta_{high}-\theta_{low}$. Assume $d\lambda$ and $d\theta$ are equivalent for $\mathcal{S}$ and $\mathcal{S}'$. Every point in the originating set, $s \in \mathcal{S}$, has an associated transition probability to $\mathcal{S}'$, $P(\mathcal{S}'|s)$. The maximum difference between transition probabilities within the set is:
%     \begin{equation}
%         \Delta P_{max}=\max_{s_1,s_2\in \mathcal{S}} |P(\mathcal{S}'|s_1) - P(\mathcal{S}'|s_2)|.
%     \end{equation}
%     As the discretization step sizes go to zero, this difference must also go to zero:
%     \begin{equation}
%         \lim_{d\lambda \to 0, d\theta\to 0} \Delta P_{max} = 0.
%     \end{equation}
% \end{theorem}
% The proof of Theorem~\ref{theorem} is in the extended version of this work~\cite{Theurkauf2022}.


\subsubsection{Scalability}

A naive method of covariance discretization could involve setting ranges on the individual elements of the covariance matrix, rather than relying on the spectral decomposition. 
% While attractive in its simplicity, that approach exacerbates an existing problem with discretization: state explosion. Consider an analogous definition of a region as some range of values over a single element of the covariance matrix. 
The full MDP state could then be described as a combination of regions across each element of the covariance matrix. Since the covariance matrix is symmetric, the number of regions, $N_R$, required to describe a state is 
$N_R = n(n+1)/2,$ where $n$ is the dimension of the state space. Whereas the spectral decomposition requires only a single region for each axis, so the number of regions required to describe a state is simply $N_R = n$.

Now assume that each matrix element is discretized into $d$ regions, and similarly that each axis in the spectral decomposition is also discretized into $d$ regions. The total number of combinations across all the regions is $d^{N_R}$. While this number explodes for both cases, it explodes less rapidly for the discretization based on the spectral decomposition. 
If we assume the same discretization at every waypoint, the total number of MDP states is then $Nd^{N_R}+3$. While this is a worst case scenario (in practice, not every combination of regions is occupied), the described techniques do suffer from a state explosion problem, which is particularly troublesome as the dimensionality of the system increases.
Finally, the spectral decomposition also benefits from visual interpretability; it is easy to visualize the uncertainty of the system in terms of vectors defining a covariance ellipse. 


% Now assume that each matrix element is discretized into $d$ regions, and similarly that each axis in the spectral decomposition is also discretized into $d$ regions. The total number of combinations across all the regions is $d^{N_R}$. While this number explodes for both cases, it explodes less rapidly for the discretization based on the spectral decomposition. If we assume the same discretization at every waypoint, the total number of states is then $Nd^{N_R}+3$. While this is a worst case scenario (in practice, not every combination of regions is occupied), the described techniques do suffer from a state explosion problem, which is particularly troublesome as the dimensionality of the system increases.

% The number of required regions for the matrix elements could be reduced by adding constraints inherent to the covariance, like positive definiteness and orthogonality. However, interpreting these constraints in matrix form is not straightforward, while they are very simple to implement in a spectral decomposition. The spectral decomposition also benefits from visual interpretability; it is easy to visualize the uncertainty of the system in terms of vectors defining a covariance ellipse. 

Off the shelf tools are available to solve the multi-objective problem on an MDP \cite{Kwiatkowska2011}. These use value iteration to construct a Pareto Front \cite{Forejt2012}, from which specific strategies are generated through linear programming \cite{Etessami2007}. The MDP analysis algorithms are polynomial with the size of the MDP.



==> sections/preliminaries.tex <==
\subsection{Gaussian Belief Assumption}
\at{I don't like this section. It upsets me.}

\at{Need to look at TAC paper, have Gaussain assumption stuff in there?}
If a trigger occurs at every time step, the filter reduces to a Kalman Filter (KF), where the belief is Gaussian and fully described by mean $\hat{x}_k$ and covariance $P_k$. However, the exact belief with the inclusion of implicit information is not necessarily Gaussian.  Work \cite{Wu2013} shows that this belief can be approximated by a Gaussian distribution that permits recursive state estimation through approximate KF. This approximation yields accurate results. 
% for a sufficiently well-tuned innovation threshold $\delta$. 
% Nonetheless, the `best' choice of $\delta$ is situation dependent and there are no established techniques for algorithmically selecting or adjusting $\delta$ in order to provide formal guarantees on performance. 

\subsection{ET Filter Equations}
The update filter equations are given below: 
\begin{enumerate}
    \item A Priori Update
    \begin{equation}
        \hat{x}_k^- = F\hat{x}_{k-1} + Gu_{k-1}
    \end{equation}
    \begin{equation}
        P_k^- = FP_{k-1}F^T + Q
    \end{equation}
    \item A Posteriori Update
    \begin{equation}
        \hat{x}_k = \hat{x}_k^- + \gamma_kK_kz_k
    \end{equation}
    \begin{equation}
        P_k = \gamma_kg_{\lambda=1}(P_k^-) + (1-\gamma_k)g_{\beta}(\delta)(P_k^-),
    \end{equation}
\end{enumerate}
where the Kalman gain $K_k$ is defined as
\begin{equation}
    K_k = P_k^-H^T[HP_k^-H^T + R]^{-1},
\end{equation}
the covariance update equation is defined as
\begin{equation}
    g_{\lambda}(P) = P - \lambda PH^T[HPH^T+R]^{-1}CP,
\end{equation}
and $\beta$ and $Q$ are defined as
\begin{equation}
    \beta(\delta) = \frac{2}{\sqrt{2\pi}}\delta\exp{-\frac{\delta^2}{2}}[1-2Q(\delta)]^{-1}
\end{equation}

\begin{equation}
    Q(\delta) \triangleq \int_{\delta}^{+\infty} \frac{1}{\sqrt{2\pi}} \exp{-\frac{x^2}{2}}dx.
\end{equation}

\begin{comment}
\subsubsection{Eigendecomposition of the Covariance Matrix}
Consider a state space system of dimension $n$. The state estimation covariance, $P$, under both KF and ET-KF techniques is an $n \times n$ matrix.  Because the covariance is a symmetric matrix, we can decompose it using its eigenvalues and eigenvectors as follows:
\begin{equation}
    P = V\Lambda V^T
\end{equation}
where $V\in \mathbb{R}^{n\times n}$ is the matrix formed by the eigenvectors, $V=[\vec{v}_1, ..., \vec{v}_n]$, and $\Delta \in \mathbb{R}^{n\times n}$ is the matrix formed with the eigenvalues on the diagonal elements, $\Lambda=diag( [\lambda_1, ..., \lambda_n] )$. The geometric interpretation of this is an ellipse with the orientation of the axes defined by the eigenvectors and the magnitude of the axes defined by the associated eigenvalues. Figure \ref{covEll} contains an example of a 2-dimensional ellipse with semi-major axis described by $\lambda_1v_1$ and semi-minor axis described by $\lambda_2v_2$. These two describing vectors can be represented as points in space, shown as stars in Figure \ref{covEll}, we will use this point representation of vectors in future figures. The symmetry of the covariance matrix implies that the eigenvectors form an orthogonal set.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{CovEllipse.pdf}
    \caption{Example Covariance Ellipse}
    \label{covEll}
    \vspace{0mm}
\end{figure}
\end{comment}


==> sections/problem.tex <==
% problem.tex

We consider an active agent communicating with a resource-limited remote sensor network. 
%that have limited resources. 
% These remote sensors have limited resources, and so it is necessary to consider how to trade off the full system's performance with conserving energy on the part of the sensors. 
The nearest sensor to the agent is able to make and communicate measurements of the agent's state to improve its performance, but the communication comes at a resource cost. %The agent can use this measurement to improve its performance. 
This setup can apply to many types of measurements, e.g.  remote one-way ranging measurements from beacons whose battery energy and data volume must be conserved in austere environments. 
% The active agent in our scenario traverses some trajectory to get to a goal state. We assume remote sensors are distributed around this trajectory and that only the nearest one is in range at a time. Under these conditions, 
The goal is to find a communication strategy to optimally trade-off sensor resource costs and agent task performance.


%% System Model %%
\subsection{System Model}
\label{subsec:SysModel}
The active agent evolves according to linear dynamics, %given by
\begin{equation}
    \label{eq:system dynamics}
    x_{k+1} = F x_k + G u_k + w_k, \quad w_k \sim \mathcal{N}(0,Q),
\end{equation}
where $x_k\in X \subseteq \mathbb{R}^n$ and $u_k\in U\subseteq\mathbb{R}^p$ are the state and input, respectively, with $F\in\mathbb{R}^{n\times n}$ and $G\in\mathbb{R}^{n\times p}$. Random process noise $w_k \in \reals^n$ is modeled as white Gaussian noise with %a random variable with a zero-mean Gaussian distribution and 
covariance $Q\in\mathbb{R}^{n\times n}$.
The initial agent state $x_0 \sim \mathcal{N}(\hat{x}_0,P_0)$ is assumed Gaussian distributed, with mean $\hat{x}_0 \in \mathbb{R}^n$ and covariance $P_0 \in \mathbb{R}^{n \times n}$. 
%
%The measurement of the agent's state is performed by the 
%\emph{nearest} remote sensor and is given by
The \emph{nearest} remote sensor measures the agent state as
\begin{equation}
    \label{eq:system measurement}
    y_k = Hx_k + v_k,\quad v_k \sim \mathcal{N}(0,R),
\end{equation}
where $y_k\in Y\subseteq\mathbb{R}^m$ is the measurement with $H\in\mathbb{R}^{m\times n}$. Random measurement noise $v_k \in \reals^m$ is also modeled as white Gaussian noise with %a random variable with a zero-mean, Gaussian distribution and
covariance $R\in\mathbb{R}^{m\times m}$. 
%
We assume the system is both \emph{controllable} and \emph{observable}, and that the noise %process and measurement noise %terms have non-degenerate distributions, i.e.,
covariance matrices $Q$ and $R$ are positive definite.
%Furthermore, 
For ease of presentation, we assume the agent %has no local sensor, meaning that the only measurements it 
only has access to measurement data from the nearest remote sensor. The extension to include local measurements is trivial.

%% State Estimation %%
\subsection{Event-Triggered State Estimation}
\label{subsec:etest}


Since sensors are resource limited, the agent uses an event triggered (ET) state estimator for efficient information sharing. %for efficient sharing of information by only communicating when it is deemed useful.
% Limiting communication  is valuable for systems with limited resources; communication can consume scarce battery power, or take up bandwidth that could be used for other information. 
When a measurement $y_k$ is taken, the sensor determines whether to report $y_k$ to the agent. This decision is based on a shared estimate of $x_k$ provided by some central estimator, e.g., the agent.  
We specifically focus on innovation-based ET described in \cite{Wu2013} although many other triggers exist \cite{Trimpe2015}. %Figure \ref{fig:EstimationDiagram} shows a block diagram of this setup. 

Let $\gamma_k \in \{0,1\}$ be the indicator for measurement communication at time $k$, where $\gamma_k = 1$ if the measurement is sent, and $\gamma_k = 0$ otherwise. Define $\I_k = (I_1, \ldots, I_k)$, $k \in \naturals$, as the sequence of available \emph{information} up to time $k$, where %at each time $1 \leq j \leq k$, 
% $I_j$ is a set containing a vector of measurements if $\gamma_j=1$, or the empty set if $\gamma_j=0$, i.e.,
\begin{equation}
    I_j = \begin{cases}
    \{y_j\} & \text{if $\gamma_j=1$}\\
    \emptyset & \text{otherwise.}
    \end{cases}, \ \mbox{for } 1 \leq j \leq k.
\end{equation}
% Note that because the exact state of the system is unknown, 
Information $\I_k$ is used to reason over the probability distribution of $x_k$.
% , represented as a probability density function. 
This distribution is denoted by $b_k$ and is referred to as the \emph{belief}, i.e., 
\begin{equation}
    x_k \sim b_k = \P(x_k \mid x_0, \mathcal{I}_k), \label{eq:beldef}
\end{equation}
and the set of all beliefs is denoted by $\beliefs$. 

Under the assumption that $\P(x_k \mid x_0, \mathcal{I}_{k-1})$ is Gaussian, work \cite{Wu2013} introduces an ET Minimum Mean Square Error (MMSE) estimator,
% According to the assumptions in \cite{Wu2013}, the ET belief is assumed (approximated) to be Gaussian and an approximate MMSE estimator derived. 
where the belief is fully described by its mean and covariance.
The expected value of the state based on the belief is the MMSE \textit{state estimate}. Before a measurement occurs, the \emph{a priori} (predicted) state estimate and error $e_k^-$ covariance at time $k$ are given by
\begin{align}
    &\hat{x}_k^-=\mathbb{E}[x_k \mid \mathcal{I}_{k-1}], \quad 
    e_k^{-}=x_k - \hat{x}_k^{-}, \\ 
     &P_k^{-} = \mathbb{E}[e_k^{-} e^{-T}_k \mid \mathcal{I}_{k-1}].
\end{align}
%%with error $e_k^-$ and covariance $P_k^-$ given by
%%\begin{equation}
%%    e_k^{-}=x_k - \hat{x}_k^{-}, \quad P_k^{-} = %\mathbb{E}[e_k^{-} e^{-T}_k \mid \mathcal{I}_{k-1}].
%%\end{equation}
After a measurement occurs, the \emph{a posteriori} (updated) estimate and error $e_k$ covariance are, for any choice of $\gamma_k$,
\begin{align}
    &\hat{x}_k = \mathbb{E}[x_k \mid \mathcal{I}_k], \label{eq:postmeandef} \quad
     e_k = x_k - \hat{x}_k, \\
    &P_k = \mathbb{E}[e_k e_k^T \mid \mathcal{I}_k] \label{eq:postcovdef}.
\end{align}
%with error $e_k$ and covariance $P_k$ given by
%\begin{equation}
%    e_k = x_k - \hat{x}_k, \quad P_k = \mathbb{E}[e_k e_k^T \mid \mathcal{I}_k].
%\end{equation}
% These estimates may be obtained through a recursive Kalman filter approximation for innovation-based ET, such that (\ref{eq:postmeandef})-(\ref{eq:postcovdef}) are functions of the innovation trigger threshold. 
% See \cite{Wu2013} for the detailed equations of this ET filter. 
In innovation-based ET, $\gamma_k$ is determined based on the measurement innovation,
$z_k = y_k - \mathbb{E}[y_k \mid \mathcal{I}_{k-1}],$
which is a Gaussian random vector with covariance $Z_k = R + HP_k^- H^T$. %Since $Z_k$ is symmetric (hence diagonalizable), a linear transformation can be defined in the form 
Let $\mathcal{F}_k = V_k \Lambda^{-1/2}_k$, where the columns of $V_k \in \reals^{n\times n}$ are the orthonormal eigenvectors of $Z_k$, and $\Lambda_k\in\mathbb{R}^{n\times n}$ is the diagonal eigenvalue matrix of $Z_k$, %. Matrix $\mathcal{F}_k$ is known as the \textit{Mahalanobis transform}, such that %and decorrelates the innovation $z_k$, i.e., 
so that the covariance of $\epsilon_k = \mathcal{F}_k z_k$ is the identity matrix. The triggering condition is then defined in terms of a given threshold $\delta \in \mathbb{R}_{>0}$ as, %when the infinity norm of the whitened measurement innovation exceeds a given threshold $\delta \in \mathbb{R}_{>0}$, i.e.,
\begin{equation}
    \gamma_k = 
    \begin{cases}
    0 & \text{if $\|\epsilon_k\|_\infty\leq\delta$}\\
    1 & \text{otherwise}.
    \end{cases}
\end{equation}
This corresponds to assessing how `surprising' $y_k$ is. For small $\delta$, many measurements are surprising, and many triggers (communications) occur; for large $\delta$, fewer measurements are surprising and thus fewer are communicated. 
As such, (\ref{eq:postmeandef}) and (\ref{eq:postcovdef}) can be obtained through a recursive Kalman filter approximation, which attenuates the Kalman gain as a function of $\delta$ when $\gamma_k=0$; see \cite{Wu2013} for complete details of this ET Kalman filter, which produces a standard Kalman update if $\gamma_k = 1$ or $\delta=0$. %; it has explicit information of the measurement at time $k$ (i.e., $I_k = \{y_k\}$) to compute the \textit{a posteriori} distribution. 
The key advantage of the ET filter is when $\gamma_k = 0$ (i.e., $I_k = \emptyset$), since the agent can still extract `implicit' information from the fact that $\|\epsilon_k\|_\infty\leq\delta$. This can be used to compute a more accurate \textit{a posteriori} estimate than the one obtained simply by keeping an unmodified \emph{a priori} estimate from the Kalman prediction step. 
%even though no measurement is available. That is, the agent estimator can use the fact that $\delta$, which can be used to compute a more accurate \textit{a posteriori} estimate than the one obtained in the predict step.

Under ET estimation, the agent's task performance and sensor resource consumption now depend on the choice of $\delta$. 
However, there are no established methods to algorithmically select or adjust $\delta$ to provide collective formal guarantees on task performance and resource consumption effects. %agent's performance. 
In this work, we design a strategy for choosing ET thresholds 
% from a given set of candidates 
% $$\Delta = \{\delta_1,\delta_2,\ldots, \delta_{n_{|\Delta|}}\}$$
over the course of the agent's trajectory to achieve an optimal resource-performance trade-off.

%% Control Laws %%
\subsection{Task and Control Laws}
\label{subsec:controlLaws}

The agent's task is to follow a nominal trajectory to a target region while avoiding unsafe states (e.g. obstacles). 
Assume the trajectory is provided via a sequence of waypoints $\wpSet = (\wp_0, \ldots, \wp_N)$ such that at $\wp_i \in \mathbb{R}^n$, for each $i\in \{0,..,N\}$, %is the point that the agent switches communication from one sensor to the next, i.e. 
the nearest sensor to the agent changes. % at point $\wp_i$. 
Such waypoints can be easily obtained, e.g. using a motion planner followed by a Voronoi segmentation with respect to the sensor network. 
Hence, the waypoints are the decision points where the triggering threshold for the next sensor (and thus the corresponding trajectory segment) is determined. 
% While the method of obtaining the waypoints is not relevant to the methods described here, in the context of a remote sensor network, where the agent communicates only with the closest sensor, the waypoints can be chosen as the points on a trajectory where the system switches from one sensor to the next. The system is controlled by a series of control laws connecting the waypoints of the discretized trajectory. 


To follow the trajectory, the agent is equipped with a series of (feedback) control laws connecting the waypoints in $\wpSet$, coupled with a termination condition that determines when to switch to the next controller.
Let $\bar{u}_i: X \times \wpSet \to U$ be the controller that drives the agent from waypoint $\wp_{i-1}$ to $\wp_{i}$ and $\zeta_i: X \times \wpSet \times \naturals \to \{0,1\}$ be the corresponding termination condition.  Then, the agent applies control law $\bar{u}_i$ until $\zeta_i$ is triggered.  We design $\zeta_i$ to trigger as %the agent sufficiently converges to $\wp_i$ or a maximum duration of time is spent, i.e., 
\begin{equation}
    \label{eq:meanConvCond}
    \zeta_i(\hat{x}_k, \wp_i, k_i) = 
    \begin{cases}
        1 & \text{if } \|\hat{x}_k - \wp_i\|_2 \leq \tol_x \text{ or } k_{i} \geq k_{\max}\\
        0 & \text{otherwise,}
    \end{cases}
\end{equation}
where $\tol_x \in\mathbb{R}_{>0}$ is the convergence tolerance, $k_{i}$ is time duration since switching to $\bar{u}_i$, and $k_{\max}$ is the max time duration threshold. 
% Once $\zeta_i$ triggers, the agent switches to controller $\bar{u}_{i+1}$ to reach waypoint $\wp_{i+2}$ with terminal condition $\zeta_{i+1}$.
% We additionally set a time-out condition, $k\geq k_{max}$, should \eqref{eq:meanConvCond} prove too strict to satisfy, where $k_{max} \in \mathbb{N}$ is the maximum number of iterations. 
% \ml{explain this better}
% This convergence criteria is the basis of the state definition in section \ref{sec:Methodologies}; it allows for a spatial discretization of the mean of the belief state. All belief states that do not satisfy the convergence criteria, i.e., when the system times out, are grouped in a catchall state. In practice, we have found that the system never reaches this time out condition if the controller is well chosen.
% \at{not sure this fits here, feels like it should go in the methodology section, but I need something to explain what happens when you time out...}
The only requirement on $\bar{u}_i$ is to drive the agent to 
proximity of $\wp_i$.
% within the defined tolerance. 
It can, for instance, consist of a reachability and a stabilizing controller using the LQG control architecture described in \cite{AghaMohammadi2014,Lahijanian2018}.
% The methods for finding the optimal tradeoffs described in this paper are agnostic to the choice of controller, but this choice can have a marked effect on the overall performance of the objectives themselves. 
% For instance, We found good results when using the linear quadratic regulator (LQG) control architecture based on \cite{AghaMohammadi2014}.
% The proposed resource-performance trade-off framework in this paper is agnostic to the choice of $\bar{u}_i$, but this choice can have a marked effect on the overall performance of the objectives themselves. 

\begin{comment}
\at{cut the rest of this paragraph?} The controller, $\bar{U}_i=(\bar{u}_{i,r},\bar{u}_{i,s})$, consists of a concatenation of a reachability controller, $\bar{u}_r$, and a stabilizing controller, $\bar{u}_s$. The reachability controller is a time-varying LQG controller that tracks a nominal trajectory. The stabilizing controller is a time-invariant LQG designed for a single point, $\wp_i$. If the reachability controller is insufficient to achieve the termination condition, then the stabilizing controller can stabilize the system about $\wp_i$ until \eqref{eq:meanConvCond} is met. 

\end{comment}


%% Objectives %%
\subsection{Resource and Performance Objectives}
\label{subsec:objFunc}
We seek to choose ET thresholds at waypoints in $\wpSet$ to achieve an optimal resource-performance trade-off.
Let $\Delta = \{\delta_1,\delta_2,\ldots, \delta_{n_{|\Delta|}}\}$ be a set of ET threshold candidates, and $\mathcal{D}(\Delta)$ be the set of all probability distributions over $\Delta$.
% A \emph{strategy} chooses thresholds from $\Delta\subset\mathbb{R}_{>0}$ at each waypoint. 
We define an \textit{ET strategy} $\strategy: \mathbb{B} \rightarrow \mathcal{D}(\Delta)$ to be a function that maps a belief $b_k \in \mathbb{B}$ at a waypoint to a probability distribution over $\Delta$.
% Recall that the choice of ET threshold directly influences the behavior of the agent. 
We want to compute $\strategy$ according to the following three competing objectives: 
(O1) minimize the probability of visiting an unsafe state (obstacle), (O2) maximize the probability of reaching the target region, and (O3) minimize resource consumption.  We refer to (O1) and (O2) as the performance objective and (O3) as the resource objective. We now formalize (O1)-(O3) as a function of $\strategy$.

Given $\strategy$, $b_k$ itself is a random variable before agent deployment due to the stochasticity of $y_k$.
To provide guarantees prior to deployment, we express the objectives based on the \emph{expected belief} defined as:
\begin{align}
    \label{eq: expected belief}
    \textbf{b}_k(\strategy) &= \mathbb{E}_Y(b_k \mid x_0, y_{0:k}, \strategy) \\
    &= \int_{y_{0:k}} \P(x_k \mid x_0, y_{0:k}, \strategy) pr(y_{0:k})dy \nonumber \\
    &= \P(x_k \mid x_0, \strategy) \nonumber
\end{align}
% \at{must figure out how to make this line up...}.The strategy is a function of the belief;  different strategies yield different choices of $\delta$, and $\delta$ in turn shapes how the belief evolves.

Consider a set of $M$ obstacles (unsafe states) $\mathcal{O}=\{X_{O_1}, ..., X_{O_M}\}$, where $X_{O_i} \subset X$ for every $i \in \{1,...,M\}$. 
% We assume that collisions with obstacles are terminal, so the portion of a belief in collision remains so for the duration of the trajectory. 
% Consequentially, we need only to examine the belief at the terminal time, $k_T$, to determine the total probability of collision. The probability of collision with a single obstacle for a given strategy is defined as:
Assuming that collisions with obstacles are terminal, the probability of collision with obstacle $X_{O_i}$ under $\strategy$ is 
\begin{equation*}
    \prob_{\coll,i}(\strategy) = pr(x_{0:k_T} \in X_{O_i}  \mid \strategy) = \int_{X_{O_i}} \hspace{-2mm} \textbf{b}_{k_T} (\strategy) dx_{k_T},
\end{equation*}
where $k_T$ is the termination time of traversing trajectory $\wpSet$.
Then, for (O1), the total probability of collision is the sum of the probabilities over all the individual obstacles,
\begin{equation}
    \prob_{\coll}(\strategy) = pr(x_{0:k_T} \in \mathcal{O} \mid \strategy) = \sum_{i=1}^{M} \prob_{\coll,i}(\strategy).
\end{equation}
% where $x_{0:k_T}$ is the sequence of states in a trajectory. 
Similarly, for (O2), the probability of ending in the target region $X_{\tar} \subset X$ is given by
\begin{equation}
    \prob_{\tar}(\strategy) = pr(x_{k_T} \in X_{\tar} \mid \strategy) = \int_{X_{\tar}} \hspace{-2mm} \textbf{b}_{k_{T}} (\strategy) dx_{k_T}.
\end{equation}

% While the resource consumption objective can be general, in this work, we focus on the energy consumed by communicating measurements. Let $c_m$ denote the fixed cost of communicating a measurement.   

For (O3), the resource cost can generally be defined as a function of the $x$, $u$, and $\delta$. For ease of presentation, we define this cost solely based on the energy consumed by communicating measurements, but the extension to include controls is straightforward. 
% The decision variable $\delta_k\in\Delta\subset\mathbb{R}_{>0}$, is a stochastic random variable with distribution given by the strategy, $\delta_k\sim\strategy(b_k)$. 
The instantaneous communication cost at time $k$ is $c_m\gamma_k$, where $c_m \in \reals_{\geq 0}$. The expected $\gamma_k$ is a function of $\delta$, i.e. $\bar{\gamma}_k(\delta) = \mathbb{E}[\gamma_k]$. 
%\begin{equation}
    %\gamma(\delta) = \mathbb{E}[\gamma_k].
%\end{equation}
Then, the expected total cost over a trajectory is
\begin{equation}
    % C_E(\strategy) = \sum_{k=0}^{k_T} \left[ \sum_{\delta \in \Delta} \Omega_{\textbf{b}_k}(\delta)c_m\gamma(\delta) \right],
    C_E(\strategy) = \sum_{k=0}^{k_T}  \sum_{\delta \in \Delta} \strategy(\textbf{b}_k)(\delta) \, c_m\bar{\gamma}_k(\delta).
\end{equation}
% where $k_T$ is the total number of time steps.
% , and $\Omega_{\textbf{b}_k}$ is strategy evaluated at $\textbf{b}_k$ (resulting in a distribution over $\delta$).


% Note that because we focus on conserving the resources of the remote sensors, the cost is based solely on the energy consumption of the sensors for communication, and the motion of the agent and any other costs are not included. However, other costs could easily be included in this framework.

\subsection{Problem Statement}
We consider the following problem: 
given a system model as described in Section \ref{subsec:SysModel}, a set of obstacles $\mathcal{O}$, a target region $X_{\tar}$, waypoints $\wpSet$, controllers as defined in Section \ref{subsec:controlLaws}, and a set of ET thresholds $\Delta$, compute optimal ET strategy $\strategy^*$ such that
\begin{equation}
    \label{eq: pareto optimal}
    \strategy^* = \argmin_{\strategy}\big(C_E(\strategy), \prob_{\coll}(\strategy), 1-\prob_{\tar}(\strategy) \big),
\end{equation}
where $\min$ is a simultaneous minimization of every element. 
%
% Recall that the strategy $\strategy$ maps to a distribution over the event triggering threshold, $\delta\in D$. Each $\strategy^*$ corresponds to the minimizing points for the objectives: $(C_E^* = E(\strategy^*), P_{tar}^* = P_{tar}(\strategy^*), P_{coll}^*=P_{coll}(\strategy^*))$. Our approach allows for the computation of all optimal tradeoffs, called the Pareto Front. For any single optimal point on the Pareto Front, we obtain the corresponding optimal strategy.

Note that \eqref{eq: pareto optimal} is a multi-objective optimization problem, and since the objectives are (often) competing, there may not exist a single solution that simultaneously optimizes each objective.  For this reason, we study the optimal trade-offs between the objectives.  Specifically, we aim to find the set of all optimal trade-offs  (Pareto front). Then, given a point from this set, we synthesize the corresponding $\strategy^*$.

% there may be infinitely many optimal values for $\min_\strategy (C_E(\strategy), P_{coll}(\strategy), P_{tar} (\strategy) )$.  That is because the objectives are competing and 
% Our approach allows for the computation of all optimal tradeoffs, called the Pareto Front. For any single optimal point on the Pareto Front, we obtain the corresponding optimal strategy.

It is exceedingly difficult to directly calculate the set of all trade-offs for a continuous system.  We instead approach this problem by constructing an abstraction of the continuous system as a finite MDP.  Multi-objective optimization algorithms are well established for MDPs and implemented in tools such as PRISM \cite{Kwiatkowska2011}, which we use for our analysis.

==> sections/problemFinal.tex <==
% problem.tex

We consider an active agent communicating with a resource-limited remote sensor network. The nearest sensor to the agent is able to make and communicate measurements of the agent's state, but communication comes at a resource cost. This setup can apply to many types of measurements, e.g.,  remote one-way ranging measurements for a mobile robot from beacons whose battery energy and data volume must be conserved in austere environments. The goal is to find a communication strategy to optimally trade-off sensor resource costs and agent task performance.

%% System Model %%
\subsection{System Model}
\label{subsec:SysModel}
The active agent evolves according to linear dynamics, %given by
\begin{equation}
    \label{eq:system dynamics}
    x_{k+1} = F x_k + G u_k + w_k, \quad w_k \sim \mathcal{N}(0,Q),
\end{equation}
where $x_k\in X \subseteq \mathbb{R}^n$ and $u_k\in U\subseteq\mathbb{R}^p$ are the state and input, respectively, with $F\in\mathbb{R}^{n\times n}$ and $G\in\mathbb{R}^{n\times p}$. Random process noise $w_k \in \reals^n$ is modeled as white Gaussian noise with %a random variable with a zero-mean Gaussian distribution and 
covariance $Q\in\mathbb{R}^{n\times n}$.
The initial agent state $x_0 \sim \mathcal{N}(\hat{x}_0,P_0)$ is assumed Gaussian distributed, with mean $\hat{x}_0 \in \mathbb{R}^n$ and covariance $P_0 \in \mathbb{R}^{n \times n}$. 
%
%The measurement of the agent's state is performed by the 
%\emph{nearest} remote sensor and is given by
The \emph{nearest} remote sensor measures the agent state as
\begin{equation}
    \label{eq:system measurement}
    y_k = Hx_k + v_k,\quad v_k \sim \mathcal{N}(0,R),
\end{equation}
where $y_k\in Y\subseteq\mathbb{R}^m$ is the measurement with $H\in\mathbb{R}^{m\times n}$. Random measurement noise $v_k \in \reals^m$ is also modeled as white Gaussian noise with %a random variable with a zero-mean, Gaussian distribution and
covariance $R\in\mathbb{R}^{m\times m}$. 
%
We assume the system is both \emph{controllable} and \emph{observable}, and that the noise %process and measurement noise %terms have non-degenerate distributions, i.e.,
covariance matrices $Q$ and $R$ are positive definite. For ease of presentation, we assume the agent only has access to measurement data from the nearest remote sensor. The extension to include local measurements is trivial.

%% State Estimation %%
\subsection{Event-Triggered State Estimation}
\label{subsec:etest}

Since the sensors are resource limited, the agent uses an event triggered (ET) state estimator for efficient information sharing. When a measurement $y_k$ is taken, the sensor determines whether to report $y_k$ to the agent. This decision is based on a shared estimate of $x_k$ provided by some central estimator, e.g., the agent. We specifically focus on innovation-based ET described in \cite{Wu2013}.

Let $\gamma_k \in \{0,1\}$ be the indicator for measurement communication at time $k$, where $\gamma_k = 1$ if the measurement is sent, and $\gamma_k = 0$ otherwise. Define $\I_k = (I_1, \ldots, I_k)$, $k \in \naturals$, as the sequence of available \emph{information} up to time $k$, where %at each time $1 \leq j \leq k$, 
% $I_j$ is a set containing a vector of measurements if $\gamma_j=1$, or the empty set if $\gamma_j=0$, i.e.,
\begin{equation}
    I_j = \begin{cases}
    \{y_j\} & \text{if $\gamma_j=1$}\\
    \emptyset & \text{otherwise.}
    \end{cases}, \ \mbox{for } 1 \leq j \leq k.
\end{equation}
% Note that because the exact state of the system is unknown, 
Information $\I_k$ is used to reason over the probability distribution of $x_k$. This distribution is denoted by $b_k$ and is referred to as the \emph{belief}, i.e., 
\begin{equation}
    x_k \sim b_k = \P(x_k \mid x_0, \mathcal{I}_k), \label{eq:beldef}
\end{equation}
with the set of all beliefs denoted by $\beliefs$. 

Under the assumption that $\P(x_k \mid x_0, \mathcal{I}_{k-1})$ is Gaussian, work \cite{Wu2013} introduces an ET Minimum Mean Square Error (MMSE) estimator, where the belief is Gaussian. The expected value of the state based on the belief is the MMSE \textit{state estimate}. Before a measurement occurs, the \emph{a priori} (predicted) state estimate and error $e_k^-$ covariance at time $k$ are given by
\begin{align}
    &\hat{x}_k^-=\mathbb{E}[x_k \mid \mathcal{I}_{k-1}], \quad 
    e_k^{-}=x_k - \hat{x}_k^{-}, \\ 
     &P_k^{-} = \mathbb{E}[e_k^{-} e^{-T}_k \mid \mathcal{I}_{k-1}].
\end{align}
%%with error $e_k^-$ and covariance $P_k^-$ given by
%%\begin{equation}
%%    e_k^{-}=x_k - \hat{x}_k^{-}, \quad P_k^{-} = %\mathbb{E}[e_k^{-} e^{-T}_k \mid \mathcal{I}_{k-1}].
%%\end{equation}
After a measurement occurs, the \emph{a posteriori} (updated) estimate and error $e_k$ covariance are, for any choice of $\gamma_k$,
\begin{align}
    &\hat{x}_k = \mathbb{E}[x_k \mid \mathcal{I}_k], \label{eq:postmeandef} \quad
     e_k = x_k - \hat{x}_k, \\
    &P_k = \mathbb{E}[e_k e_k^T \mid \mathcal{I}_k] \label{eq:postcovdef}.
\end{align}
%with error $e_k$ and covariance $P_k$ given by
%\begin{equation}
%    e_k = x_k - \hat{x}_k, \quad P_k = \mathbb{E}[e_k e_k^T \mid \mathcal{I}_k].
%\end{equation}
% These estimates may be obtained through a recursive Kalman filter approximation for innovation-based ET, such that (\ref{eq:postmeandef})-(\ref{eq:postcovdef}) are functions of the innovation trigger threshold. 
% See \cite{Wu2013} for the detailed equations of this ET filter. 
In innovation-based ET, $\gamma_k$ is determined based on the measurement innovation,
$z_k = y_k - \mathbb{E}[y_k \mid \mathcal{I}_{k-1}],$
which is a Gaussian random vector with covariance $Z_k = R + HP_k^- H^T$. %Since $Z_k$ is symmetric (hence diagonalizable), a linear transformation can be defined in the form 
Let $\mathcal{F}_k = V_k \Lambda^{-1/2}_k$, where the columns of $V_k \in \reals^{n\times n}$ are the orthonormal eigenvectors of $Z_k$, and $\Lambda_k\in\mathbb{R}^{n\times n}$ is the diagonal eigenvalue matrix of $Z_k$, so that the covariance of the whittened innovation $\epsilon_k = \mathcal{F}_k z_k$ is the identity matrix. The triggering condition is then defined in terms of a given threshold $\delta \in \mathbb{R}_{>0}$ as, 
\begin{equation}
    \gamma_k = 
    \begin{cases}
    0 & \text{if $\|\epsilon_k\|_\infty\leq\delta$}\\
    1 & \text{otherwise}.
    \end{cases}
\end{equation}
This corresponds to assessing how `surprising' $y_k$ is. For small $\delta$, many measurements are surprising, and many triggers (communications) occur; and vice versa for large $\delta$. As such, (\ref{eq:postmeandef}) and (\ref{eq:postcovdef}) can be obtained through a recursive Kalman filter approximation, which attenuates the Kalman gain as a function of $\delta$ when $\gamma_k=0$, and produces a standard Kalman update if $\gamma_k = 1$ or $\delta=0$ (see \cite{Wu2013} for complete details). The key advantage of the ET filter is the `implicit' information that $\|\epsilon_k\|_\infty\leq\delta$ when $\gamma_k = 0$ (i.e., $I_k = \emptyset$). This can be used to compute a more accurate \textit{a posteriori} estimate than the one obtained simply by keeping an unmodified \emph{a priori} estimate from the Kalman prediction step. 

Under ET estimation, the agent's task performance and sensor resource consumption now depend on the choice of $\delta$. 
However, there are no established methods to algorithmically select or adjust $\delta$ to provide collective formal guarantees on task performance and resource consumption effects. This work fills that gap.

%In this work, we design a strategy for choosing ET thresholds over the course of the agent's trajectory to achieve an optimal resource-performance trade-off.

%% Control Laws %%
\subsection{Task and Control Laws}
\label{subsec:controlLaws}

The agent's task is to follow a nominal trajectory to a target region while avoiding unsafe states (e.g. obstacles). 
Assume the trajectory is provided via a sequence of waypoints $\wpSet = (\wp_0, \ldots, \wp_N)$ such that at $\wp_i \in \mathbb{R}^n$, for each $i\in \{0,..,N\}$, the nearest sensor to the agent changes. Such waypoints can be easily obtained, e.g., using a motion planner followed by a Voronoi segmentation with respect to the sensor network. 
Hence, the waypoints are the decision points where the triggering threshold for the next sensor (and thus the corresponding trajectory segment) is determined. 

To follow the trajectory, the agent is equipped with a series of (feedback) control laws connecting the waypoints in $\wpSet$, coupled with a termination condition that determines when to switch to the next controller.
Let $\mathcal{U}_i: X \times \wpSet \to U$ be the control law that drives the agent from waypoint $\wp_{i-1}$ to $\wp_{i}$ and $\zeta_i: X \times \wpSet \times \naturals \to \{0,1\}$ be the corresponding termination condition.  Then, the agent applies control law $\mathcal{U}_i$ until $\zeta_i$ is triggered.  We design $\zeta_i$ to trigger as  
\begin{equation}
    \label{eq:meanConvCond}
    \zeta_i(\hat{x}_k, \wp_i, k_i) = 
    \begin{cases}
        1 & \text{if } \|\hat{x}_k - \wp_i\|_2 \leq \tol_x \text{ or } k_{i} \geq k_{\max}\\
        0 & \text{otherwise,}
    \end{cases}
\end{equation}
where $\tol_x \in\mathbb{R}_{>0}$ is the convergence tolerance, $k_{i}$ is time duration since switching to $\mathcal{U}_i$, and $k_{\max}$ is the max time duration threshold. 
% Once $\zeta_i$ triggers, the agent switches to controller $\bar{u}_{i+1}$ to reach waypoint $\wp_{i+2}$ with terminal condition $\zeta_{i+1}$.
% We additionally set a time-out condition, $k\geq k_{max}$, should \eqref{eq:meanConvCond} prove too strict to satisfy, where $k_{max} \in \mathbb{N}$ is the maximum number of iterations. 
% \ml{explain this better}
% This convergence criteria is the basis of the state definition in section \ref{sec:Methodologies}; it allows for a spatial discretization of the mean of the belief state. All belief states that do not satisfy the convergence criteria, i.e., when the system times out, are grouped in a catchall state. In practice, we have found that the system never reaches this time out condition if the controller is well chosen.
% \at{not sure this fits here, feels like it should go in the methodology section, but I need something to explain what happens when you time out...}
The only requirement on $\mathcal{U}_i$ is to drive the agent to 
proximity of $\wp_i$.
% within the defined tolerance. 
It can, for instance, consist of a reachability and a stabilizing controller using the LQG control architecture described in \cite{AghaMohammadi2014,Lahijanian2018}.
% The methods for finding the optimal tradeoffs described in this paper are agnostic to the choice of controller, but this choice can have a marked effect on the overall performance of the objectives themselves. 
% For instance, We found good results when using the linear quadratic regulator (LQG) control architecture based on \cite{AghaMohammadi2014}.
% The proposed resource-performance trade-off framework in this paper is agnostic to the choice of $\bar{u}_i$, but this choice can have a marked effect on the overall performance of the objectives themselves. 

\begin{comment}
\at{cut the rest of this paragraph?} The controller, $\bar{U}_i=(\bar{u}_{i,r},\bar{u}_{i,s})$, consists of a concatenation of a reachability controller, $\bar{u}_r$, and a stabilizing controller, $\bar{u}_s$. The reachability controller is a time-varying LQG controller that tracks a nominal trajectory. The stabilizing controller is a time-invariant LQG designed for a single point, $\wp_i$. If the reachability controller is insufficient to achieve the termination condition, then the stabilizing controller can stabilize the system about $\wp_i$ until \eqref{eq:meanConvCond} is met. 

\end{comment}


%% Objectives %%
\subsection{Resource and Performance Objectives}
\label{subsec:objFunc}
We seek to choose ET thresholds at waypoints in $\wpSet$ to achieve an optimal resource-performance trade-off.
Let $\Delta = \{\delta_1,\delta_2,\ldots, \delta_{|\Delta|}\}$ be a set of ET threshold candidates, and $\mathcal{D}(\Delta)$ be the set of all probability distributions over $\Delta$.
% A \emph{strategy} chooses thresholds from $\Delta\subset\mathbb{R}_{>0}$ at each waypoint. 
We define an \textit{ET strategy} $\strategy: \mathbb{B} \rightarrow \mathcal{D}(\Delta)$ to be a function that maps a belief $b_k \in \mathbb{B}$ at a waypoint to a probability distribution over $\Delta$.
% Recall that the choice of ET threshold directly influences the behavior of the agent. 
We want to compute $\strategy$ according to the following three competing objectives: 
(O1) minimize the probability of visiting an unsafe state (obstacle), (O2) maximize the probability of reaching the target region, and (O3) minimize resource consumption.  We refer to (O1) and (O2) as the performance objective and (O3) as the resource objective. We now formalize (O1)-(O3) as a function of $\strategy$.

Given $\strategy$, $b_k$ itself is a random variable before agent deployment due to the stochasticity of $y_k$.
To provide guarantees prior to deployment, we express the objectives based on the \emph{expected belief} defined as:
\begin{align}
    \label{eq: expected belief}
    \textbf{b}_k(\strategy) &= \mathbb{E}_Y(b_k \mid x_0, y_{0:k}, \strategy) \\
    &= \int_{y_{0:k}} \P(x_k \mid x_0, y_{0:k}, \strategy) pr(y_{0:k})dy \nonumber \\
    &= \P(x_k \mid x_0, \strategy) \nonumber
\end{align}
% \at{must figure out how to make this line up...}.The strategy is a function of the belief;  different strategies yield different choices of $\delta$, and $\delta$ in turn shapes how the belief evolves.

Consider a set of $M$ obstacles (unsafe states) $\mathcal{O}=\{X_{O_1}, ..., X_{O_M}\}$, where $X_{O_i} \subset X$ for every $i \in \{1,...,M\}$. 
% We assume that collisions with obstacles are terminal, so the portion of a belief in collision remains so for the duration of the trajectory. 
% Consequentially, we need only to examine the belief at the terminal time, $k_T$, to determine the total probability of collision. The probability of collision with a single obstacle for a given strategy is defined as:
Assuming that collisions with obstacles are terminal, the probability of collision with obstacle $X_{O_i}$ under $\strategy$ is 
\begin{equation*}
    \prob_{\coll,i}(\strategy) = pr(x_{0:k_T} \in X_{O_i}  \mid \strategy) = \int_{X_{O_i}} \hspace{-2mm} \textbf{b}_{k_T} (\strategy) dx_{k_T},
\end{equation*}
where $k_T$ is the termination time of traversing trajectory $\wpSet$.
Then, for (O1), the total probability of collision is the sum of the probabilities over all the individual obstacles,
\begin{equation}
    \prob_{\coll}(\strategy) = pr(x_{0:k_T} \in \mathcal{O} \mid \strategy) = \sum_{i=1}^{M} \prob_{\coll,i}(\strategy).
\end{equation}
% where $x_{0:k_T}$ is the sequence of states in a trajectory. 
Similarly, for (O2), the probability of ending in the target region $X_{\tar} \subset X$ is given by
\begin{equation}
    \prob_{\tar}(\strategy) = pr(x_{k_T} \in X_{\tar} \mid \strategy) = \int_{X_{\tar}} \hspace{-2mm} \textbf{b}_{k_{T}} (\strategy) dx_{k_T}.
\end{equation}

For (O3), the resource cost can generally be defined as a function of $x$, $u$, and $\delta$. For ease of presentation, we define this cost solely based on the energy consumed by communicating measurements, but extending to include actuation, or anything else, is straightforward. The instantaneous communication cost at time $k$ is $c_m\gamma_k$, where $c_m \in \reals_{\geq 0}$. The expected $\gamma_k$ is a function of $\delta$, i.e. $\bar{\gamma}_k(\delta) = \mathbb{E}[\gamma_k]$. Then, the expected total cost over a trajectory is
\begin{equation}
    C_E(\strategy) = \sum_{k=0}^{k_T}  \sum_{\delta \in \Delta} \strategy(\textbf{b}_k)(\delta) \, c_m\bar{\gamma}_k(\delta).
\end{equation}
% where $k_T$ is the total number of time steps.
% , and $\Omega_{\textbf{b}_k}$ is strategy evaluated at $\textbf{b}_k$ (resulting in a distribution over $\delta$).


% Note that because we focus on conserving the resources of the remote sensors, the cost is based solely on the energy consumption of the sensors for communication, and the motion of the agent and any other costs are not included. However, other costs could easily be included in this framework.

\subsection{Problem Statement}
We consider the following problem: 
given a system model as described in Section \ref{subsec:SysModel}, a set of obstacles $\mathcal{O}$, a target region $X_{\tar}$, waypoints $\wpSet$, controllers as defined in Section \ref{subsec:controlLaws}, and a set of ET thresholds $\Delta$, compute optimal ET strategy $\strategy^*$ such that
\begin{equation}
    \label{eq: pareto optimal}
    \strategy^* = \arg \min_{\strategy}\big(C_E(\strategy), \prob_{\coll}(\strategy), 1-\prob_{\tar}(\strategy) \big),
\end{equation}
where $\min$ is a simultaneous minimization of every element. 

Note that \eqref{eq: pareto optimal} is a multi-objective optimization problem, and since the objectives are (often) competing, there may not exist a single solution that simultaneously optimizes each objective.  For this reason, we study the set of all optimal trade-offs between the objectives (Pareto front). Then, given a point from this set, we synthesize the corresponding $\strategy^*$.

It is computationally intractable to directly calculate the set of all trade-offs for a continuous system. We instead approach this problem by constructing an abstraction of the continuous system as a finite MDP. Established algorithms for multi-objective optimization of MDPs are polynomial with the size of the MDP and implemented in tools such as PRISM \cite{Kwiatkowska2011}, which we use for our analysis.
